Submodular Benchmark Selection

Evaluating a new language model means running it on a large, growing collection of benchmarks, at considerable cost. Much of this cost is redundant: arranged as a matrix of models by benchmarks, scores are strongly correlated and concentrate in a few dimensions, so a few well-chosen benchmarks largely determine the rest. This allows us to run a new model on a few benchmarks and predict the rest with a simple Gaussian model that copes with missing scores. The key question is \emph{which few to run}. An answer comes from sensor placement, which chooses the observations that carry the most information, measured by entropy or mutual information. We argue that the objective should instead reward a selection for how well it predicts every benchmark. This leads to two coverage objectives: explained variance, the predictions' accuracy if the estimated correlations were exact, and facility location, which credits each benchmark with its best proxy among the selected ones. On eleven score matrices built from public evaluation results, the coverage objectives predict the scores of held-out models best wherever the correlations can be estimated. The information objectives fall behind because they favor benchmarks that the selection predicts poorly (entropy) or that the others predict well (mutual information), not benchmarks that predict the others. By contrast, facility location predicts practically as well as explained variance, holds up on the addition of newer models and under real costs, has classical guarantees (even under a budget), and gives readable selections.

==> cr/numbers_cmds.tex <==
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\makeatletter
\providecommand{\nv@missingstyle}[1]{%
  \begingroup\@ifundefined{textcolor}{\bfseries}{\color{red}\bfseries}#1\endgroup}
\newcommand{\nv@get}[2]{%
  \ifcsname nv@#1@#2\endcsname
    \csname nv@#1@#2\endcsname
  \else
    \PackageWarning{numbers}{Number `#2' (variant #1) undefined.
      Run paper/cr/tools/paper_numbers.sh}%
    \nv@missingstyle{??#2??}%
  \fi}
\DeclareRobustCommand{\nv}[2][]{\nv@get{v#1}{#2}}
\DeclareRobustCommand{\nvd}[2][3]{\nv@get{d#1}{#2}}
\DeclareRobustCommand{\nvneg}[2][3]{\nv@get{neg#1}{#2}}
\DeclareRobustCommand{\nvci}[2][3]{\nv@get{ci#1}{#2}}
\DeclareRobustCommand{\nvcineg}[2][3]{\nv@get{cineg#1}{#2}}
\DeclareRobustCommand{\nvdiff}[3][3]{\nv@get{diff#1}{#2-#3}}
\DeclareRobustCommand{\nvpct}[2][0]{\nv@get{pct#1}{#2}}
\DeclareRobustCommand{\nvtt}[1]{\nv@get{tt}{#1}}
\DeclareRobustCommand{\nvtext}[1]{\nv@get{text}{#1}}
\makeatother


==> cr/numbers_paper.tex <==
%
%
%
\makeatletter
\@namedef{nv@ci3@BenchFamPairDiffHelmMmluAllFaclocAwareVsBlindKfive}{[\ensuremath{-}0.011, +0.023]}
\@namedef{nv@ci3@BenchFamPairDiffHelmMmluAllFaclocBlindVsRandomKfive}{[\ensuremath{-}0.017, +0.064]}
\@namedef{nv@ci3@BenchFamPairDiffMergedAllFaclocAwareVsBlindKfive}{[\ensuremath{-}0.024, +0.191]}
\@namedef{nv@ci3@BenchFamPairDiffMergedAllFaclocBlindVsRandomKfive}{[\ensuremath{-}0.180, +0.182]}
\@namedef{nv@ci3@BenchFamPairDiffMmluAllFaclocBlindVsRandomKfive}{[+0.008, +0.021]}
\@namedef{nv@ci3@BenchFamPairDiffMtebAllFaclocAwareVsBlindKfive}{[+0.004, +0.076]}
\@namedef{nv@ci3@BenchFamPairDiffMtebAllFaclocBlindVsRandomKfive}{[\ensuremath{-}0.040, +0.023]}
\@namedef{nv@ci3@BenchFamPairDiffOlvOneItemsAllFaclocAwareVsBlindKfive}{[+0.005, +0.013]}
\@namedef{nv@ci3@BenchFamPairDiffOlvOneItemsAllFaclocBlindVsRandomKfive}{[+0.014, +0.035]}
\@namedef{nv@ci3@BenchFamPairDiffOlvTwoSubAllFaclocAwareVsBlindKfive}{[+0.046, +0.065]}
\@namedef{nv@ci3@BenchFamPairDiffOlvTwoSubAllFaclocBlindVsRandomKfive}{[\ensuremath{-}0.017, +0.057]}
\@namedef{nv@ci3@BootDiffProspMtebTraceVsFaclocKthree}{[+0.006, +0.108]}
\@namedef{nv@ci3@BootDiffProspOlvTwoSubCutJanTwentyfiveTraceVsFaclocKthree}{[+0.002, +0.010]}
\@namedef{nv@ci3@EstDiffBenchpressPairwiseFaclocKfive}{[\ensuremath{-}0.040, +0.517]}
\@namedef{nv@ci3@ItemBudgetPairDiffOlvOneItemsBenchFaclocVsItemsCenterQtwelvethousandeighthundred}{[+0.037, +0.049]}
\@namedef{nv@ci3@PairDiffBaseBenchpressFaclocVsRandomKfive}{[\ensuremath{-}0.345, +0.211]}
\@namedef{nv@ci3@PairDiffBaseEpochFaclocVsRandomKfive}{[+0.028, +0.311]}
\@namedef{nv@ci3@PairDiffBaseHelmClassicFaclocVsRandomKfive}{[\ensuremath{-}0.217, +0.462]}
\@namedef{nv@ci3@PairDiffBaseHelmLiteFaclocVsRandomKfive}{[\ensuremath{-}0.063, +0.163]}
\@namedef{nv@ci3@PairDiffBaseHelmMmluFaclocVsRandomKfive}{[+0.001, +0.078]}
\@namedef{nv@ci3@PairDiffBaseMergedFaclocVsFaclocSqKone}{[\ensuremath{-}0.382, +0.035]}
\@namedef{nv@ci3@PairDiffBaseMergedFaclocVsRandomKfive}{[\ensuremath{-}0.025, +0.128]}
\@namedef{nv@ci3@PairDiffBaseMergedVOneFaclocVsRandomKfive}{[\ensuremath{-}0.017, +0.129]}
\@namedef{nv@ci3@PairDiffBaseMmluFaclocVsRandomKfive}{[+0.020, +0.037]}
\@namedef{nv@ci3@PairDiffBaseMtebFaclocVsRandomKfive}{[\ensuremath{-}0.046, +0.092]}
\@namedef{nv@ci3@PairDiffBaseMtebTwothousandtwentysixFaclocVsRandomKfive}{[+0.024, +0.084]}
\@namedef{nv@ci3@PairDiffBaseOlvOneItemsFaclocVsFaclocSqKtwo}{[+0.001, +0.012]}
\@namedef{nv@ci3@PairDiffBaseOlvOneItemsFaclocVsRandomKfive}{[+0.020, +0.042]}
\@namedef{nv@ci3@PairDiffBaseOlvTwoSubFaclocVsRandomKfive}{[+0.064, +0.123]}
\@namedef{nv@ci3@PairDiffBenchpressFaclocVsRandomKfivePninety}{[\ensuremath{-}0.201, +0.179]}
\@namedef{nv@ci3@PairDiffEpochFaclocVsRandomKfivePninety}{[\ensuremath{-}0.159, +0.236]}
\@namedef{nv@ci3@PairDiffImpBenchpressFaclocHardVsGaussKfive}{[\ensuremath{-}0.233, +0.172]}
\@namedef{nv@ci3@PairDiffImpBenchpressFaclocSoftVsGaussKfive}{[\ensuremath{-}0.102, +0.354]}
\@namedef{nv@ci3@PairDiffImpMergedFaclocHardVsGaussKfive}{[\ensuremath{-}0.124, +0.023]}
\@namedef{nv@ci3@PairDiffImpMergedFaclocSoftVsGaussKfive}{[\ensuremath{-}0.253, \ensuremath{-}0.078]}
\@namedef{nv@ci3@PairDiffImpMmluFaclocHardVsGaussKfive}{[\ensuremath{-}0.020, \ensuremath{-}0.018]}
\@namedef{nv@ci3@PairDiffImpMmluFaclocSoftVsGaussKfive}{[\ensuremath{-}0.132, \ensuremath{-}0.121]}
\@namedef{nv@ci3@PairDiffImpMtebFaclocHardVsGaussKfive}{[\ensuremath{-}0.107, +0.004]}
\@namedef{nv@ci3@PairDiffImpMtebFaclocSoftVsGaussKfive}{[\ensuremath{-}0.144, \ensuremath{-}0.008]}
\@namedef{nv@ci3@PairDiffMergedFaclocVsRandomKfivePninety}{[\ensuremath{-}0.189, +0.179]}
\@namedef{nv@ci3@PairDiffMmluFaclocVsRandomKfivePninety}{[+0.004, +0.049]}
\@namedef{nv@ci3@PairDiffMtebFaclocVsRandomKfivePninety}{[\ensuremath{-}0.111, +0.145]}
\@namedef{nv@ci3@PairDiffMtebTwothousandtwentysixFaclocVsRandomKfivePninety}{[\ensuremath{-}0.145, +0.188]}
\@namedef{nv@ci3@PairDiffOlvTwoSubFaclocVsRandomKfivePninety}{[+0.011, +0.186]}
\@namedef{nv@ci3@StabPairDiffBenchpressFaclocAltVsFullKfive}{[\ensuremath{-}0.223, +0.216]}
\@namedef{nv@ci3@StabPairDiffMergedFaclocAltVsFullKfive}{[\ensuremath{-}0.021, +0.060]}
\@namedef{nv@ci3@StabPairDiffMergedTraceAltVsFullKfive}{[\ensuremath{-}0.031, +0.065]}
\@namedef{nv@ci3@StabPairDiffMtebFaclocAltVsFullKfive}{[\ensuremath{-}0.034, +0.037]}
\@namedef{nv@ci4@BenchFamPairDiffMmluAllFaclocAwareVsBlindKfive}{[+0.0001, +0.0018]}
\@namedef{nv@ci4@BootDiffProspOlvTwoSubMathCutMarTwentyfiveTraceVsFaclocKfive}{[+0.0003, +0.0036]}
\@namedef{nv@cineg3@BootDiffProspEpochByModelCutJanTwentyfiveTraceVsFaclocKfive}{[\ensuremath{-}0.064, +0.009]}
\@namedef{nv@cineg3@BootDiffProspEpochCutJanTwentyfiveTraceVsFaclocKfive}{[\ensuremath{-}0.094, +0.003]}
\@namedef{nv@cineg3@BootDiffProspEpochCutJanTwentysixTraceVsFaclocKfive}{[\ensuremath{-}0.388, \ensuremath{-}0.071]}
\@namedef{nv@cineg3@BootDiffProspEpochCutJulTwentyfiveTraceVsFaclocKfive}{[\ensuremath{-}0.037, \ensuremath{-}0.004]}
\@namedef{nv@cineg3@BootDiffProspEpochCutJulTwentyfourTraceVsFaclocKfive}{[+0.406, +0.828]}
\@namedef{nv@cineg3@BootDiffProspHelmTraceVsFaclocKfive}{[+0.066, +0.222]}
\@namedef{nv@cineg3@BootDiffProspMtebLateTraceVsFaclocKfive}{[\ensuremath{-}0.073, +0.005]}
\@namedef{nv@cineg3@BootDiffProspMtebTraceVsFaclocKfive}{[\ensuremath{-}0.034, +0.032]}
\@namedef{nv@cineg3@BootDiffProspOlvTwoSubCutJanTwentyfiveTraceVsFaclocKfive}{[+0.007, +0.017]}
\@namedef{nv@cineg3@BootDiffProspOlvTwoSubCutMarTwentyfiveTraceVsFaclocKfive}{[\ensuremath{-}0.005, +0.008]}
\@namedef{nv@cineg3@BootDiffProspOlvTwoSubCutOctTwentyfourTraceVsFaclocKfive}{[\ensuremath{-}0.003, +0.004]}
\@namedef{nv@cineg3@BootDiffProspOlvTwoSubMathCutJanTwentyfiveTraceVsFaclocKfive}{[+0.001, +0.009]}
\@namedef{nv@cineg3@CostFixedPairDiffMtebCheapFirstVsKnapFaclocFoneBzeropointtwo}{[+0.105, +0.274]}
\@namedef{nv@cineg3@PairDiffBaseBenchpressTraceVsFaclocKfive}{[\ensuremath{-}0.292, +0.568]}
\@namedef{nv@cineg3@PairDiffBaseEpochTraceVsFaclocKfive}{[\ensuremath{-}0.050, +0.084]}
\@namedef{nv@cineg3@PairDiffBaseHelmClassicTraceVsFaclocKfive}{[\ensuremath{-}0.386, +0.764]}
\@namedef{nv@cineg3@PairDiffBaseHelmLiteTraceVsFaclocKfive}{[\ensuremath{-}0.036, +0.020]}
\@namedef{nv@cineg3@PairDiffBaseHelmMmluTraceVsFaclocKfive}{[\ensuremath{-}0.030, +0.017]}
\@namedef{nv@cineg3@PairDiffBaseMergedTraceVsFaclocKfive}{[\ensuremath{-}0.050, +0.093]}
\@namedef{nv@cineg3@PairDiffBaseMergedVOneMiVsFaclocKfive}{[+0.037, +0.229]}
\@namedef{nv@cineg3@PairDiffBaseMergedVOneTraceVsFaclocKfive}{[\ensuremath{-}0.038, +0.084]}
\@namedef{nv@cineg3@PairDiffBaseMmluTraceVsFaclocKfive}{[\ensuremath{-}0.002, \ensuremath{-}0.001]}
\@namedef{nv@cineg3@PairDiffBaseMtebTraceVsFaclocKfive}{[\ensuremath{-}0.089, +0.043]}
\@namedef{nv@cineg3@PairDiffBaseMtebTwothousandtwentysixTraceVsFaclocKfive}{[\ensuremath{-}0.028, +0.050]}
\@namedef{nv@cineg3@PairDiffBaseOlvOneItemsTraceVsFaclocKfive}{[\ensuremath{-}0.006, +0.004]}
\@namedef{nv@cineg3@PairDiffBaseOlvTwoSubTraceVsFaclocKfive}{[\ensuremath{-}0.003, \ensuremath{-}0.001]}
\@namedef{nv@cineg3@PairDiffMmluMiVsEntropyKone}{[+0.024, +0.030]}
\@namedef{nv@d3@BenchFamPairDiffHelmMmluAllFaclocAwareVsBlindKfive}{+0.006}
\@namedef{nv@d3@BenchFamPairDiffHelmMmluAllFaclocBlindVsRandomKfive}{+0.023}
\@namedef{nv@d3@BenchFamPairDiffMergedAllFaclocAwareVsBlindKfive}{+0.084}
\@namedef{nv@d3@BenchFamPairDiffMergedAllFaclocBlindVsRandomKfive}{+0.001}
\@namedef{nv@d3@BenchFamPairDiffMmluAllFaclocBlindVsRandomKfive}{+0.015}
\@namedef{nv@d3@BenchFamPairDiffMtebAllFaclocAwareVsBlindKfive}{+0.040}
\@namedef{nv@d3@BenchFamPairDiffMtebAllFaclocBlindVsRandomKfive}{\ensuremath{-}0.009}
\@namedef{nv@d3@BenchFamPairDiffOlvOneItemsAllFaclocAwareVsBlindKfive}{+0.009}
\@namedef{nv@d3@BenchFamPairDiffOlvOneItemsAllFaclocBlindVsRandomKfive}{+0.025}
\@namedef{nv@d3@BenchFamPairDiffOlvTwoSubAllFaclocAwareVsBlindKfive}{+0.056}
\@namedef{nv@d3@BenchFamPairDiffOlvTwoSubAllFaclocBlindVsRandomKfive}{+0.020}
\@namedef{nv@d3@BootDiffProspMtebTraceVsFaclocKthree}{+0.048}
\@namedef{nv@d3@BootDiffProspOlvTwoSubCutJanTwentyfiveTraceVsFaclocKthree}{+0.006}
\@namedef{nv@d3@CostFixedPairDiffMmluKnapFaclocVsCardFaclocFoneBtwo}{+0.479}
\@namedef{nv@d3@CostFixedPairDiffMmluKnapFaclocVsCardFaclocFzeroBone}{+0.463}
\@namedef{nv@d3@CostFixedPairDiffMmluKnapFaclocVsRandomFoneBtwo}{+0.116}
\@namedef{nv@d3@CostFixedPairDiffMmluKnapFaclocVsRandomFzeroBone}{+0.129}
\@namedef{nv@d3@CostFixedPairDiffMtebKnapFaclocVsCardFaclocFoneBzeropointtwo}{+0.082}
\@namedef{nv@d3@CostFixedPairDiffMtebKnapFaclocVsCardFaclocFzeroBtwo}{+0.045}
\@namedef{nv@d3@CostFixedPairDiffMtebKnapFaclocVsRandomFoneBzeropointtwo}{+0.112}
\@namedef{nv@d3@CostFixedPairDiffMtebKnapFaclocVsRandomFzeroBtwo}{+0.045}
\@namedef{nv@d3@EstDiffBenchpressPairwiseFaclocKfive}{+0.238}
\@namedef{nv@d3@EstPairBenchpressPairwiseFaclocVsRandomKfive}{+0.062}
\@namedef{nv@d3@EstPairHiBenchpressPairwiseFaclocVsRandomKfive}{+0.222}
\@namedef{nv@d3@EstPairLoBenchpressPairwiseFaclocVsRandomKfive}{\ensuremath{-}0.098}
\@namedef{nv@d3@ItemBudgetPairDiffOlvOneItemsBenchFaclocVsItemsCenterQtwelvethousandeighthundred}{+0.043}
\@namedef{nv@d3@ObjGapMaskTrainBenchpressFaclocKfive}{\ensuremath{-}0.127}
\@namedef{nv@d3@ObjGapMaskTrainBenchpressTraceKfive}{\ensuremath{-}0.185}
\@namedef{nv@d3@ObjGapMaskTrainMergedFaclocKfive}{\ensuremath{-}0.079}
\@namedef{nv@d3@ObjGapMaskTrainMergedTraceKfive}{\ensuremath{-}0.103}
\@namedef{nv@d3@ObjGapMaskTrainMmluFaclocKfive}{\ensuremath{-}0.001}
\@namedef{nv@d3@ObjGapMaskTrainMtebFaclocKfive}{\ensuremath{-}0.013}
\@namedef{nv@d3@ObjGapMaskTrainMtebTraceKfive}{\ensuremath{-}0.011}
\@namedef{nv@d3@ObjGapTotalTrainBenchpressFaclocKfive}{\ensuremath{-}0.666}
\@namedef{nv@d3@ObjGapTotalTrainBenchpressTraceKfive}{\ensuremath{-}0.842}
\@namedef{nv@d3@ObjGapTotalTrainMergedFaclocKfive}{\ensuremath{-}0.080}
\@namedef{nv@d3@ObjGapTotalTrainMergedTraceKfive}{\ensuremath{-}0.116}
\@namedef{nv@d3@ObjGapTotalTrainMmluFaclocKfive}{\ensuremath{-}0.001}
\@namedef{nv@d3@ObjGapTotalTrainMmluTraceKfive}{\ensuremath{-}0.001}
\@namedef{nv@d3@ObjGapTotalTrainMtebFaclocKfive}{\ensuremath{-}0.079}
\@namedef{nv@d3@ObjGapTotalTrainMtebTraceKfive}{\ensuremath{-}0.059}
\@namedef{nv@d3@PairDiffBaseBenchpressFaclocVsRandomKfive}{\ensuremath{-}0.067}
\@namedef{nv@d3@PairDiffBaseEpochFaclocVsRandomKfive}{+0.169}
\@namedef{nv@d3@PairDiffBaseHelmClassicFaclocVsRandomKfive}{+0.123}
\@namedef{nv@d3@PairDiffBaseHelmLiteFaclocVsRandomKfive}{+0.050}
\@namedef{nv@d3@PairDiffBaseHelmMmluFaclocVsRandomKfive}{+0.039}
\@namedef{nv@d3@PairDiffBaseMergedFaclocVsFaclocSqKone}{\ensuremath{-}0.174}
\@namedef{nv@d3@PairDiffBaseMergedFaclocVsRandomKfive}{+0.051}
\@namedef{nv@d3@PairDiffBaseMergedVOneFaclocVsRandomKfive}{+0.056}
\@namedef{nv@d3@PairDiffBaseMmluFaclocVsRandomKfive}{+0.028}
\@namedef{nv@d3@PairDiffBaseMtebFaclocVsRandomKfive}{+0.023}
\@namedef{nv@d3@PairDiffBaseMtebTwothousandtwentysixFaclocVsRandomKfive}{+0.054}
\@namedef{nv@d3@PairDiffBaseOlvOneItemsFaclocVsFaclocSqKtwo}{+0.006}
\@namedef{nv@d3@PairDiffBaseOlvOneItemsFaclocVsRandomKfive}{+0.031}
\@namedef{nv@d3@PairDiffBaseOlvTwoSubFaclocVsRandomKfive}{+0.093}
\@namedef{nv@d3@PairDiffBenchpressFaclocVsRandomKfivePninety}{\ensuremath{-}0.011}
\@namedef{nv@d3@PairDiffEpochFaclocVsRandomKfivePninety}{+0.039}
\@namedef{nv@d3@PairDiffImpBenchpressFaclocHardVsGaussKfive}{\ensuremath{-}0.031}
\@namedef{nv@d3@PairDiffImpBenchpressFaclocSoftVsGaussKfive}{+0.126}
\@namedef{nv@d3@PairDiffImpMergedFaclocHardVsGaussKfive}{\ensuremath{-}0.050}
\@namedef{nv@d3@PairDiffImpMergedFaclocSoftVsGaussKfive}{\ensuremath{-}0.166}
\@namedef{nv@d3@PairDiffImpMmluFaclocHardVsGaussKfive}{\ensuremath{-}0.019}
\@namedef{nv@d3@PairDiffImpMmluFaclocSoftVsGaussKfive}{\ensuremath{-}0.127}
\@namedef{nv@d3@PairDiffImpMtebFaclocHardVsGaussKfive}{\ensuremath{-}0.051}
\@namedef{nv@d3@PairDiffImpMtebFaclocSoftVsGaussKfive}{\ensuremath{-}0.076}
\@namedef{nv@d3@PairDiffMergedFaclocVsRandomKfivePninety}{\ensuremath{-}0.005}
\@namedef{nv@d3@PairDiffMmluFaclocVsRandomKfivePninety}{+0.027}
\@namedef{nv@d3@PairDiffMtebFaclocVsRandomKfivePninety}{+0.017}
\@namedef{nv@d3@PairDiffMtebTwothousandtwentysixFaclocVsRandomKfivePninety}{+0.022}
\@namedef{nv@d3@PairDiffOlvTwoSubFaclocVsRandomKfivePninety}{+0.099}
\@namedef{nv@d3@PenaltyCenProspHelmFaclocKfive}{\ensuremath{-}0.311}
\@namedef{nv@d3@PenaltyProspEpochCutJulTwentyfourFaclocKfive}{+0.517}
\@namedef{nv@d3@RevMonoDatasetsMmluPairedFiveRTwoCiHigh}{+0.006}
\@namedef{nv@d3@RevMonoDatasetsMmluPairedFiveRTwoCiLow}{+0.002}
\@namedef{nv@d3@RevMonoDatasetsMmluPairedFiveRTwoMeanDiff}{+0.004}
\@namedef{nv@d3@StabPairDiffBenchpressFaclocAltVsFullKfive}{\ensuremath{-}0.004}
\@namedef{nv@d3@StabPairDiffMergedFaclocAltVsFullKfive}{+0.019}
\@namedef{nv@d3@StabPairDiffMergedTraceAltVsFullKfive}{+0.017}
\@namedef{nv@d3@StabPairDiffMtebFaclocAltVsFullKfive}{+0.001}
\@namedef{nv@d3@TokSuitePairDiffHelmClassicFaclocTokensVsFaclocInstancesBtwo}{+0.205}
\@namedef{nv@d3@TokSuitePairDiffHelmClassicFaclocTokensVsRandomBone}{+0.081}
\@namedef{nv@d3@TokSuitePairDiffHelmLiteFaclocTokensVsFaclocInstancesBtwenty}{+0.207}
\@namedef{nv@d3@TokSuitePairDiffHelmLiteFaclocTokensVsRandomBtwenty}{+0.101}
\@namedef{nv@d3@TokSuitePairDiffHelmMmluFaclocTokensVsFaclocInstancesBtwo}{+0.074}
\@namedef{nv@d3@TokSuitePairDiffHelmMmluFaclocTokensVsRandomBthirty}{+0.086}
\@namedef{nv@d4@BenchFamPairDiffMmluAllFaclocAwareVsBlindKfive}{+0.0010}
\@namedef{nv@d4@BootDiffProspOlvTwoSubMathCutMarTwentyfiveTraceVsFaclocKfive}{+0.0019}
\@namedef{nv@d4@ObjGapMaskTrainMmluTraceKfive}{\ensuremath{-}0.0004}
\@namedef{nv@diff3@RevClipDatasetsBenchpressEntropyRTwoClipListMean-RevClipDatasetsBenchpressEntropyRTwoRawListMean}{+0.193}
\@namedef{nv@diff3@RevClipDatasetsBenchpressFaclocRTwoClipListMean-RevClipDatasetsBenchpressFaclocRTwoRawListMean}{+0.067}
\@namedef{nv@diff3@RevClipDatasetsMtebEntropyRTwoClipListMean-RevClipDatasetsMtebEntropyRTwoRawListMean}{+0.005}
\@namedef{nv@diff3@RsqBaseHelmLiteEntropyKfive-RsqBaseHelmLiteTraceKfive}{+0.002}
\@namedef{nv@diff3@RsqFamEpochFaclocKfive-RsqBaseEpochFaclocKfive}{\ensuremath{-}0.106}
\@namedef{nv@diff3@RsqFamHelmClassicFaclocKfive-RsqBaseHelmClassicFaclocKfive}{+0.141}
\@namedef{nv@diff3@RsqFamHelmLiteFaclocKfive-RsqBaseHelmLiteFaclocKfive}{\ensuremath{-}0.337}
\@namedef{nv@diff3@RsqFamHelmMmluFaclocKfive-RsqBaseHelmMmluFaclocKfive}{\ensuremath{-}0.031}
\@namedef{nv@diff3@RsqFamMergedFaclocKfive-RsqBaseMergedFaclocKfive}{+0.048}
\@namedef{nv@diff3@RsqFamMmluFaclocKfive-RsqBaseMmluFaclocKfive}{\ensuremath{-}0.020}
\@namedef{nv@diff3@RsqFamMtebFaclocKfive-RsqBaseMtebFaclocKfive}{\ensuremath{-}0.147}
\@namedef{nv@diff3@RsqFamMtebTwothousandtwentysixFaclocKfive-RsqBaseMtebTwothousandtwentysixFaclocKfive}{\ensuremath{-}0.162}
\@namedef{nv@diff3@RsqFamOlvOneItemsFaclocKfive-RsqBaseOlvOneItemsFaclocKfive}{\ensuremath{-}0.023}
\@namedef{nv@diff3@RsqFamOlvTwoSubFaclocKfive-RsqBaseOlvTwoSubFaclocKfive}{\ensuremath{-}0.010}
\@namedef{nv@diff4@RsqFamBenchpressFaclocKfive-RsqBaseBenchpressFaclocKfive}{+0.0003}
\@namedef{nv@neg3@BootDiffProspEpochByModelCutJanTwentyfiveTraceVsFaclocKfive}{\ensuremath{-}0.025}
\@namedef{nv@neg3@BootDiffProspEpochCutJanTwentyfiveTraceVsFaclocKfive}{\ensuremath{-}0.047}
\@namedef{nv@neg3@BootDiffProspEpochCutJanTwentysixTraceVsFaclocKfive}{\ensuremath{-}0.278}
\@namedef{nv@neg3@BootDiffProspEpochCutJulTwentyfiveTraceVsFaclocKfive}{\ensuremath{-}0.019}
\@namedef{nv@neg3@BootDiffProspEpochCutJulTwentyfourTraceVsFaclocKfive}{+0.596}
\@namedef{nv@neg3@BootDiffProspHelmTraceVsFaclocKfive}{+0.137}
\@namedef{nv@neg3@BootDiffProspMtebLateTraceVsFaclocKfive}{\ensuremath{-}0.033}
\@namedef{nv@neg3@BootDiffProspMtebTraceVsFaclocKfive}{+0.007}
\@namedef{nv@neg3@BootDiffProspOlvTwoSubCutJanTwentyfiveTraceVsFaclocKfive}{+0.012}
\@namedef{nv@neg3@BootDiffProspOlvTwoSubCutMarTwentyfiveTraceVsFaclocKfive}{+0.002}
\@namedef{nv@neg3@BootDiffProspOlvTwoSubCutOctTwentyfourTraceVsFaclocKfive}{+0.001}
\@namedef{nv@neg3@BootDiffProspOlvTwoSubMathCutJanTwentyfiveTraceVsFaclocKfive}{+0.005}
\@namedef{nv@neg3@CostFixedPairDiffMmluCheapFirstVsKnapFaclocFoneBtwo}{+0.020}
\@namedef{nv@neg3@CostFixedPairDiffMmluCheapFirstVsKnapFaclocFzeroBtwenty}{+0.008}
\@namedef{nv@neg3@CostFixedPairDiffMmluKnapMiVsKnapFaclocFoneBtwenty}{+0.029}
\@namedef{nv@neg3@CostFixedPairDiffMmluKnapMiVsKnapFaclocFzeroBone}{+0.027}
\@namedef{nv@neg3@CostFixedPairDiffMmluKnapTraceVsKnapFaclocFoneBeight}{\ensuremath{-}0.005}
\@namedef{nv@neg3@CostFixedPairDiffMmluKnapTraceVsKnapFaclocFzeroBfive}{\ensuremath{-}0.006}
\@namedef{nv@neg3@CostFixedPairDiffMtebCheapFirstVsKnapFaclocFoneBzeropointtwo}{+0.190}
\@namedef{nv@neg3@CostFixedPairDiffMtebCheapFirstVsKnapFaclocFzeroBtwo}{+0.024}
\@namedef{nv@neg3@CostFixedPairDiffMtebKnapMiVsKnapFaclocFoneBzeropointtwo}{+0.125}
\@namedef{nv@neg3@CostFixedPairDiffMtebKnapMiVsKnapFaclocFzeroBtwenty}{+0.009}
\@namedef{nv@neg3@CostFixedPairDiffMtebKnapTraceVsKnapFaclocFoneBtwo}{+0.005}
\@namedef{nv@neg3@CostFixedPairDiffMtebKnapTraceVsKnapFaclocFzeroBtwo}{+0.010}
\@namedef{nv@neg3@PairDiffBaseBenchpressTraceVsFaclocKfive}{+0.138}
\@namedef{nv@neg3@PairDiffBaseEpochTraceVsFaclocKfive}{+0.017}
\@namedef{nv@neg3@PairDiffBaseHelmClassicTraceVsFaclocKfive}{+0.189}
\@namedef{nv@neg3@PairDiffBaseHelmLiteTraceVsFaclocKfive}{\ensuremath{-}0.008}
\@namedef{nv@neg3@PairDiffBaseHelmMmluTraceVsFaclocKfive}{\ensuremath{-}0.006}
\@namedef{nv@neg3@PairDiffBaseMergedTraceVsFaclocKfive}{+0.022}
\@namedef{nv@neg3@PairDiffBaseMergedVOneMiVsFaclocKfive}{+0.133}
\@namedef{nv@neg3@PairDiffBaseMergedVOneTraceVsFaclocKfive}{+0.023}
\@namedef{nv@neg3@PairDiffBaseMmluTraceVsFaclocKfive}{\ensuremath{-}0.001}
\@namedef{nv@neg3@PairDiffBaseMtebTraceVsFaclocKfive}{\ensuremath{-}0.023}
\@namedef{nv@neg3@PairDiffBaseMtebTwothousandtwentysixTraceVsFaclocKfive}{+0.011}
\@namedef{nv@neg3@PairDiffBaseOlvOneItemsTraceVsFaclocKfive}{\ensuremath{-}0.001}
\@namedef{nv@neg3@PairDiffBaseOlvTwoSubTraceVsFaclocKfive}{\ensuremath{-}0.002}
\@namedef{nv@neg3@PairDiffMmluMiVsEntropyKone}{+0.027}
\@namedef{nv@neg3@TokSuitePairDiffHelmClassicTraceTokensVsFaclocTokensBtwo}{+0.010}
\@namedef{nv@neg3@TokSuitePairDiffHelmLiteTraceTokensVsFaclocTokensBtwenty}{+0.036}
\@namedef{nv@neg3@TokSuitePairDiffHelmMmluTraceTokensVsFaclocTokensBone}{\ensuremath{-}0.054}
\@namedef{nv@pct0@FillTestCtrlMteb}{72\%}
\@namedef{nv@pct0@FillTestProspMteb}{44\%}
\@namedef{nv@pct0@ItemBudgetFixedOverheadShareOlvOneItemsItemsCfiftyQeighthundred}{94\%}
\@namedef{nv@pct0@ItemBudgetFixedOverheadShareOlvOneItemsItemsCtenQonehundredten}{82\%}
\@namedef{nv@pct0@ObjBruteMergedFaclocKthreeFRatioMin}{96\%}
\@namedef{nv@pct0@ObjFirstBenchpressMiPLowShare}{96\%}
\@namedef{nv@pct0@ObjFirstBenchpressTracePLowShare}{69\%}
\@namedef{nv@pct0@ObjFirstMergedMiPLowShare}{98\%}
\@namedef{nv@pct0@ObjFirstMergedTracePLowShare}{4\%}
\@namedef{nv@pct0@ObjFirstMmluMiPLowShare}{95\%}
\@namedef{nv@pct0@ObjFirstMmluTracePLowShare}{95\%}
\@namedef{nv@pct0@ObjFirstMtebMiPLowShare}{90\%}
\@namedef{nv@pct0@ObjFirstMtebTracePLowShare}{54\%}
\@namedef{nv@pct0@ObjFlVsTraceSharedBenchpressKfive}{36\%}
\@namedef{nv@pct0@ObjFlVsTraceSharedMergedKfive}{21\%}
\@namedef{nv@pct0@ObjFlVsTraceSharedMmluKfive}{80\%}
\@namedef{nv@pct0@ObjFlVsTraceSharedMtebKfive}{66\%}
\@namedef{nv@pct0@ObjTheoryBenchpressTraceIncreaseFrac}{14\%}
\@namedef{nv@pct0@ObjTheoryMergedTraceIncreaseFrac}{13\%}
\@namedef{nv@pct0@ObjTheoryMmluMiKepsRel}{16\%}
\@namedef{nv@pct0@ObjTheoryMmluMiNonmonotone}{100\%}
\@namedef{nv@pct0@ObjTheoryMmluTraceIncreaseFrac}{10\%}
\@namedef{nv@pct0@ObjTheoryMtebMiKepsRel}{29\%}
\@namedef{nv@pct0@ObjTheoryMtebMiNonmonotone}{100\%}
\@namedef{nv@pct0@ObjTheoryMtebTraceIncreaseFrac}{13\%}
\@namedef{nv@pct0@RevContamMergedDrawsConfigsFracZeropointoneDeltaZeropointoneMiTopFiveAfterFrac}{50\%}
\@namedef{nv@pct0@RevContamMergedDrawsConfigsFracZeropointthreeDeltaZeropointtwoMiTopFiveAfterFrac}{5\%}
\@namedef{nv@pct0@RevContamMtebDrawsConfigsFracZeropointthreeDeltaZeropointtwoEntropyTopFiveAfterFrac}{90\%}
\@namedef{nv@pct0@StabSubFracMerged}{80\%}
\@namedef{nv@pct1@ObjBruteMergedFaclocKthreeFRatio}{98.8\%}
\@namedef{nv@pct1@ObjBruteMtebTraceKthreeFRatio}{97.7\%}
\@namedef{nv@text@SelMmluFaclocKfivePickFive}{abstract algebra}
\@namedef{nv@text@SelMmluFaclocKfivePickFour}{college mathematics}
\@namedef{nv@text@SelMmluFaclocKfivePickOne}{professional psychology}
\@namedef{nv@text@SelMmluFaclocKfivePickThree}{miscellaneous}
\@namedef{nv@text@SelMmluFaclocKfivePickTwo}{elementary mathematics}
\@namedef{nv@tt@RevContamBenchmark}{\texttt{miscellaneous}}
\@namedef{nv@tt@RevContamMergedBenchmark}{\texttt{arena\_\allowbreak{}hard/\allowbreak{}score}}
\@namedef{nv@tt@RevContamMtebBenchmark}{\texttt{BiorxivClusteringS2S}}
\@namedef{nv@v0@CostFixedMedianCostMmlu}{173}
\@namedef{nv@v0@EstNCellsBenchpressFaclocKfive}{14}
\@namedef{nv@v0@EstNCellsMergedFaclocKfive}{16}
\@namedef{nv@v0@ItemBudgetFixedCrossQSigStayOlvOneItemsBenchFaclocVsItemsCenterCfifty}{150}
\@namedef{nv@v0@ItemBudgetFixedCrossQSigStayOlvOneItemsBenchFaclocVsItemsCenterConehundred}{200}
\@namedef{nv@v0@ItemBudgetFixedCrossQSigStayOlvOneItemsBenchFaclocVsItemsCenterCten}{110}
\@namedef{nv@v0@ItemBudgetFixedCrossQSigStayOlvOneItemsBenchFaclocVsItemsCenterCtwohundred}{300}
\@namedef{nv@v0@ItemBudgetFixedCrossQSigStayOlvOneItemsBenchFaclocVsItemsCenterCzero}{800}
\@namedef{nv@v0@NModelsProspEpochCutJulTwentyfourFaclocKfive}{65}
\@namedef{nv@v0@NModelsProspEpochCutJulTwentyfourTraceKfive}{12}
\@namedef{nv@v0@NModelsProspMtebFaclocKfive}{50}
\@namedef{nv@v0@NModelsProspMtebHubKfive}{24}
\@namedef{nv@v0@RevContamDrawsConfigsFracZeropointthreeDeltaZeropointtwoEntropyRankAfterMedian}{10}
\@namedef{nv@v0@RevContamDrawsConfigsFracZeropointthreeDeltaZeropointtwoFaclocRankAfterMedian}{14}
\@namedef{nv@v1@CostFixedMedianCostMteb}{32{,}078.5}
\@namedef{nv@v1@DataBenchpressObsPct}{33.8}
\@namedef{nv@v1@DataEpochObsPct}{17.7}
\@namedef{nv@v1@DataHelmClassicObsPct}{81.7}
\@namedef{nv@v1@DataHelmLiteObsPct}{99.9}
\@namedef{nv@v1@DataHelmMmluObsPct}{100.0}
\@namedef{nv@v1@DataMergedObsPct}{31.2}
\@namedef{nv@v1@DataMergedVOneObsPct}{31.1}
\@namedef{nv@v1@DataMmluObsPct}{100.0}
\@namedef{nv@v1@DataMtebObsPct}{77.3}
\@namedef{nv@v1@DataMtebTwothousandtwentysixObsPct}{72.4}
\@namedef{nv@v1@DataOlvOneItemsObsPct}{100.0}
\@namedef{nv@v1@DataOlvTwoSubObsPct}{100.0}
\@namedef{nv@v2@FaclocCoverMergedKten}{0.82}
\@namedef{nv@v2@FaclocCoverMmluKten}{0.97}
\@namedef{nv@v2@JaccFamBenchpressFaclocKfive}{0.14}
\@namedef{nv@v2@JaccFamEpochFaclocKfive}{0.35}
\@namedef{nv@v2@JaccFamHelmClassicFaclocKfive}{0.58}
\@namedef{nv@v2@JaccFamHelmLiteFaclocKfive}{0.94}
\@namedef{nv@v2@JaccFamHelmMmluFaclocKfive}{0.64}
\@namedef{nv@v2@JaccFamMergedFaclocKfive}{0.15}
\@namedef{nv@v2@JaccFamMmluFaclocKfive}{1.00}
\@namedef{nv@v2@JaccFamMtebFaclocKfive}{0.88}
\@namedef{nv@v2@JaccFamMtebTwothousandtwentysixFaclocKfive}{0.93}
\@namedef{nv@v2@JaccFamOlvOneItemsFaclocKfive}{0.87}
\@namedef{nv@v2@JaccFamOlvTwoSubFaclocKfive}{0.89}
\@namedef{nv@v2@NormMmluWMedian}{0.84}
\@namedef{nv@v2@NormMtebWMedian}{0.89}
\@namedef{nv@v2@ObjFlVsTraceJaccBenchpressKfive}{0.24}
\@namedef{nv@v2@ObjFlVsTraceJaccMergedKfive}{0.12}
\@namedef{nv@v2@ObjFlVsTraceJaccMmluKfive}{0.67}
\@namedef{nv@v2@ObjFlVsTraceJaccMtebKfive}{0.51}
\@namedef{nv@v2@ObjModalFirstMergedMiRestRsq}{0.95}
\@namedef{nv@v2@ObjRedundBenchpressEntropyKfive}{0.27}
\@namedef{nv@v2@ObjRedundBenchpressFaclocKfive}{0.42}
\@namedef{nv@v2@ObjRedundBenchpressHubKfive}{0.80}
\@namedef{nv@v2@ObjRedundBenchpressMiKfive}{0.39}
\@namedef{nv@v2@ObjRedundBenchpressPcaKfive}{0.29}
\@namedef{nv@v2@ObjRedundBenchpressRandomKfive}{0.47}
\@namedef{nv@v2@ObjRedundBenchpressTraceKfive}{0.42}
\@namedef{nv@v2@ObjRedundMergedEntropyKfive}{0.21}
\@namedef{nv@v2@ObjRedundMergedFaclocKfive}{0.40}
\@namedef{nv@v2@ObjRedundMergedHubKfive}{0.80}
\@namedef{nv@v2@ObjRedundMergedMiKfive}{0.28}
\@namedef{nv@v2@ObjRedundMergedPcaKfive}{0.22}
\@namedef{nv@v2@ObjRedundMergedRandomKfive}{0.48}
\@namedef{nv@v2@ObjRedundMergedTraceKfive}{0.35}
\@namedef{nv@v2@ObjRedundMmluEntropyKfive}{0.66}
\@namedef{nv@v2@ObjRedundMmluFaclocKfive}{0.71}
\@namedef{nv@v2@ObjRedundMmluHubKfive}{0.98}
\@namedef{nv@v2@ObjRedundMmluMiKfive}{0.89}
\@namedef{nv@v2@ObjRedundMmluPcaKfive}{0.63}
\@namedef{nv@v2@ObjRedundMmluRandomKfive}{0.87}
\@namedef{nv@v2@ObjRedundMmluTraceKfive}{0.70}
\@namedef{nv@v2@ObjRedundMtebEntropyKfive}{0.45}
\@namedef{nv@v2@ObjRedundMtebFaclocKfive}{0.74}
\@namedef{nv@v2@ObjRedundMtebHubKfive}{0.94}
\@namedef{nv@v2@ObjRedundMtebMiKfive}{0.70}
\@namedef{nv@v2@ObjRedundMtebPcaKfive}{0.45}
\@namedef{nv@v2@ObjRedundMtebRandomKfive}{0.71}
\@namedef{nv@v2@ObjRedundMtebTraceKfive}{0.68}
\@namedef{nv@v2@ObjSpearmanBenchpressEntropyKfive}{\ensuremath{-}0.08}
\@namedef{nv@v2@ObjSpearmanBenchpressFaclocKfive}{0.01}
\@namedef{nv@v2@ObjSpearmanBenchpressFaclocKone}{0.20}
\@namedef{nv@v2@ObjSpearmanBenchpressHubKfive}{0.14}
\@namedef{nv@v2@ObjSpearmanBenchpressMiKfive}{\ensuremath{-}0.20}
\@namedef{nv@v2@ObjSpearmanBenchpressMiKone}{\ensuremath{-}0.02}
\@namedef{nv@v2@ObjSpearmanBenchpressTraceKfive}{0.01}
\@namedef{nv@v2@ObjSpearmanBenchpressTraceKone}{0.18}
\@namedef{nv@v2@ObjSpearmanMergedEntropyKfive}{\ensuremath{-}0.09}
\@namedef{nv@v2@ObjSpearmanMergedFaclocKfive}{0.31}
\@namedef{nv@v2@ObjSpearmanMergedFaclocKone}{0.28}
\@namedef{nv@v2@ObjSpearmanMergedHubKfive}{0.12}
\@namedef{nv@v2@ObjSpearmanMergedMiKone}{\ensuremath{-}0.03}
\@namedef{nv@v2@ObjSpearmanMergedTraceKfive}{0.29}
\@namedef{nv@v2@ObjSpearmanMergedTraceKone}{0.35}
\@namedef{nv@v2@ObjSpearmanMmluEntropyKfive}{0.56}
\@namedef{nv@v2@ObjSpearmanMmluFaclocKfive}{0.81}
\@namedef{nv@v2@ObjSpearmanMmluFaclocKone}{0.98}
\@namedef{nv@v2@ObjSpearmanMmluHubKfive}{\ensuremath{-}0.58}
\@namedef{nv@v2@ObjSpearmanMmluMiKfive}{0.29}
\@namedef{nv@v2@ObjSpearmanMmluMiKone}{0.84}
\@namedef{nv@v2@ObjSpearmanMmluTraceKfive}{0.97}
\@namedef{nv@v2@ObjSpearmanMmluTraceKone}{0.98}
\@namedef{nv@v2@ObjSpearmanMtebEntropyKfive}{0.23}
\@namedef{nv@v2@ObjSpearmanMtebFaclocKfive}{0.38}
\@namedef{nv@v2@ObjSpearmanMtebFaclocKone}{0.73}
\@namedef{nv@v2@ObjSpearmanMtebHubKfive}{\ensuremath{-}0.06}
\@namedef{nv@v2@ObjSpearmanMtebMiKfive}{0.24}
\@namedef{nv@v2@ObjSpearmanMtebMiKone}{0.46}
\@namedef{nv@v2@ObjSpearmanMtebTraceKfive}{0.48}
\@namedef{nv@v2@ObjSpearmanMtebTraceKone}{0.74}
\@namedef{nv@v2@ObjTheoryBenchpressTraceGamma}{0.71}
\@namedef{nv@v2@ObjTheoryBenchpressTraceGammaBound}{0.51}
\@namedef{nv@v2@ObjTheoryBenchpressTraceGammaBoundMin}{0.40}
\@namedef{nv@v2@ObjTheoryMergedTraceGamma}{0.76}
\@namedef{nv@v2@ObjTheoryMergedTraceGammaBound}{0.53}
\@namedef{nv@v2@ObjTheoryMmluTraceGamma}{0.91}
\@namedef{nv@v2@ObjTheoryMmluTraceGammaBound}{0.60}
\@namedef{nv@v2@ObjTheoryMtebTraceGamma}{0.82}
\@namedef{nv@v2@ObjTheoryMtebTraceGammaBound}{0.56}
\@namedef{nv@v2@RevMonoDatasetsMergedPairedFiveMiMeanDiff}{0.24}
\@namedef{nv@v2@RevMonoDatasetsMmluMinGain}{0.10}
\@namedef{nv@v2@RevMonoDatasetsMtebPairedFiveMiMeanDiff}{0.36}
\@namedef{nv@v2@StabCrossJaccMergedFaclocKfive}{0.18}
\@namedef{nv@v2@StabCrossJaccMmluFaclocKfive}{1.00}
\@namedef{nv@v2@StabJaccPairBenchpressFaclocKfive}{0.09}
\@namedef{nv@v2@StabJaccPairMergedFaclocKfive}{0.14}
\@namedef{nv@v2@StabJaccPairMergedTraceKfive}{0.10}
\@namedef{nv@v2@StabJaccPairMmluFaclocKfive}{0.98}
\@namedef{nv@v2@StabJaccPairMtebFaclocKfive}{0.47}
\@namedef{nv@v2@TokSpearmanHelmClassic}{0.33}
\@namedef{nv@v2@TokSpearmanHelmLite}{0.14}
\@namedef{nv@v2@TokSpearmanHelmMmlu}{0.83}
\@namedef{nv@v3@ObjSpearmanMergedMiKfive}{\ensuremath{-}0.002}
\@namedef{nv@v4@EstMaxAbsDiffMmluPsdFloorFaclocKfive}{0.0003}
\@namedef{nv@v4@RsqFamBenchpressTraceKfive}{0.0002}
\@namedef{nv@v@BenchFamNFamMeanMerged}{9}
\@namedef{nv@v@BenchFamNFamMerged}{10}
\@namedef{nv@v@BenchFamRsqHelmMmluAllFaclocAwareKfive}{0.747}
\@namedef{nv@v@BenchFamRsqHelmMmluAllFaclocBlindKfive}{0.741}
\@namedef{nv@v@BenchFamRsqHelmMmluAllMiBlindKfive}{0.741}
\@namedef{nv@v@BenchFamRsqHelmMmluAllRandomKfive}{0.717}
\@namedef{nv@v@BenchFamRsqHelmMmluAllTraceBlindKfive}{0.755}
\@namedef{nv@v@BenchFamRsqMergedAllFaclocAwareKfive}{0.367}
\@namedef{nv@v@BenchFamRsqMergedAllFaclocBlindKfive}{0.284}
\@namedef{nv@v@BenchFamRsqMergedAllMiBlindKfive}{0.251}
\@namedef{nv@v@BenchFamRsqMergedAllRandomKfive}{0.283}
\@namedef{nv@v@BenchFamRsqMergedAllTraceBlindKfive}{0.303}
\@namedef{nv@v@BenchFamRsqMmluAllFaclocAwareKfive}{0.902}
\@namedef{nv@v@BenchFamRsqMmluAllFaclocBlindKfive}{0.901}
\@namedef{nv@v@BenchFamRsqMmluAllMiBlindKfive}{0.896}
\@namedef{nv@v@BenchFamRsqMmluAllRandomKfive}{0.886}
\@namedef{nv@v@BenchFamRsqMmluAllTraceBlindKfive}{0.904}
\@namedef{nv@v@BenchFamRsqMtebAllFaclocAwareKfive}{0.707}
\@namedef{nv@v@BenchFamRsqMtebAllFaclocBlindKfive}{0.668}
\@namedef{nv@v@BenchFamRsqMtebAllMiBlindKfive}{0.680}
\@namedef{nv@v@BenchFamRsqMtebAllRandomKfive}{0.676}
\@namedef{nv@v@BenchFamRsqMtebAllTraceBlindKfive}{0.689}
\@namedef{nv@v@BenchFamRsqOlvOneItemsAllFaclocAwareKfive}{0.839}
\@namedef{nv@v@BenchFamRsqOlvOneItemsAllFaclocBlindKfive}{0.830}
\@namedef{nv@v@BenchFamRsqOlvOneItemsAllMiBlindKfive}{0.834}
\@namedef{nv@v@BenchFamRsqOlvOneItemsAllRandomKfive}{0.805}
\@namedef{nv@v@BenchFamRsqOlvOneItemsAllTraceBlindKfive}{0.832}
\@namedef{nv@v@BenchFamRsqOlvTwoSubAllFaclocAwareKfive}{0.611}
\@namedef{nv@v@BenchFamRsqOlvTwoSubAllFaclocBlindKfive}{0.555}
\@namedef{nv@v@BenchFamRsqOlvTwoSubAllMiBlindKfive}{0.546}
\@namedef{nv@v@BenchFamRsqOlvTwoSubAllRandomKfive}{0.535}
\@namedef{nv@v@BenchFamRsqOlvTwoSubAllTraceBlindKfive}{0.565}
\@namedef{nv@v@CostFixedEmptyMmluFoneBone}{50}
\@namedef{nv@v@CostFixedPairDiffMmluCheapFirstVsKnapFaclocFzeroBthree}{0.006}
\@namedef{nv@v@CostFixedPairDiffMmluKnapTraceVsKnapFaclocFzeroBfive}{0.006}
\@namedef{nv@v@CostFixedSigNegMmluCheapFirstVsKnapFaclocFzero}{4}
\@namedef{nv@v@CostFixedSigPosMmluCheapFirstVsKnapFaclocFzero}{3}
\@namedef{nv@v@CostFixedSigPosMmluKnapTraceVsKnapFaclocFzero}{6}
\@namedef{nv@v@CostFixedSigPosMtebKnapFaclocVsRandomFzero}{2}
\@namedef{nv@v@CostMaxMmlu}{1{,}534}
\@namedef{nv@v@CostMaxMteb}{8{,}848{,}803}
\@namedef{nv@v@CostMinMmlu}{100}
\@namedef{nv@v@CostMinMteb}{100}
\@namedef{nv@v@CostRsqMmluCardFaclocBone}{0.373}
\@namedef{nv@v@CostRsqMmluKnapFaclocBone}{0.836}
\@namedef{nv@v@CostRsqMmluRandomBone}{0.707}
\@namedef{nv@v@CoverMmluFaclocKfivePickOne}{27}
\@namedef{nv@v@CoverMmluFaclocKfivePickThree}{21}
\@namedef{nv@v@CoverMmluFaclocKfivePickTwo}{4}
\@namedef{nv@v@DataBenchpressM}{83}
\@namedef{nv@v@DataBenchpressN}{49}
\@namedef{nv@v@DataEpochM}{277}
\@namedef{nv@v@DataEpochN}{61}
\@namedef{nv@v@DataHelmClassicM}{67}
\@namedef{nv@v@DataHelmClassicN}{16}
\@namedef{nv@v@DataHelmLiteM}{91}
\@namedef{nv@v@DataHelmLiteN}{10}
\@namedef{nv@v@DataHelmMmluM}{79}
\@namedef{nv@v@DataHelmMmluN}{57}
\@namedef{nv@v@DataMergedM}{118}
\@namedef{nv@v@DataMergedN}{114}
\@namedef{nv@v@DataMergedVOneM}{118}
\@namedef{nv@v@DataMergedVOneN}{114}
\@namedef{nv@v@DataMmluM}{5{,}452}
\@namedef{nv@v@DataMmluN}{57}
\@namedef{nv@v@DataMtebM}{263}
\@namedef{nv@v@DataMtebN}{56}
\@namedef{nv@v@DataMtebTwothousandtwentysixM}{333}
\@namedef{nv@v@DataMtebTwothousandtwentysixN}{56}
\@namedef{nv@v@DataOlvOneItemsM}{395}
\@namedef{nv@v@DataOlvOneItemsN}{62}
\@namedef{nv@v@DataOlvTwoSubM}{4{,}493}
\@namedef{nv@v@DataOlvTwoSubN}{42}
\@namedef{nv@v@EigKMergedVarninety}{8}
\@namedef{nv@v@EigKMmluVarninety}{2}
\@namedef{nv@v@EigKMtebVarninety}{6}
\@namedef{nv@v@EstMaxAbsDiffMtebFaclocKfive}{0.034}
\@namedef{nv@v@EstRsqBenchpressAlphaPointOneFaclocKfive}{0.105}
\@namedef{nv@v@EstRsqBenchpressAlphaPointOneMiKfive}{0.107}
\@namedef{nv@v@EstRsqBenchpressAlphaPointOneRandomKfive}{0.183}
\@namedef{nv@v@EstRsqBenchpressAlphaPointOneTraceKfive}{0.124}
\@namedef{nv@v@EstRsqBenchpressAlphaPointThreeFaclocKfive}{0.153}
\@namedef{nv@v@EstRsqBenchpressAlphaPointThreeMiKfive}{0.152}
\@namedef{nv@v@EstRsqBenchpressAlphaPointThreeRandomKfive}{0.195}
\@namedef{nv@v@EstRsqBenchpressAlphaPointThreeTraceKfive}{0.182}
\@namedef{nv@v@EstRsqBenchpressDefaultFaclocKfive}{0.053}
\@namedef{nv@v@EstRsqBenchpressDefaultMiKfive}{\ensuremath{-}0.059}
\@namedef{nv@v@EstRsqBenchpressDefaultRandomKfive}{0.120}
\@namedef{nv@v@EstRsqBenchpressDefaultTraceKfive}{\ensuremath{-}0.085}
\@namedef{nv@v@EstRsqBenchpressEligTenFaclocKfive}{0.133}
\@namedef{nv@v@EstRsqBenchpressEligTenMiKfive}{\ensuremath{-}0.058}
\@namedef{nv@v@EstRsqBenchpressEligTenRandomKfive}{0.205}
\@namedef{nv@v@EstRsqBenchpressEligTenTraceKfive}{0.102}
\@namedef{nv@v@EstRsqBenchpressPairwiseFaclocKfive}{0.291}
\@namedef{nv@v@EstRsqBenchpressPairwiseMiKfive}{0.059}
\@namedef{nv@v@EstRsqBenchpressPairwiseRandomKfive}{0.230}
\@namedef{nv@v@EstRsqBenchpressPairwiseTraceKfive}{0.301}
\@namedef{nv@v@EstRsqBenchpressTolLooseFaclocKfive}{0.210}
\@namedef{nv@v@EstRsqBenchpressTolLooseMiKfive}{0.006}
\@namedef{nv@v@EstRsqBenchpressTolLooseRandomKfive}{0.150}
\@namedef{nv@v@EstRsqBenchpressTolLooseTraceKfive}{0.147}
\@namedef{nv@v@EstRsqBenchpressTolTightFaclocKfive}{\ensuremath{-}0.137}
\@namedef{nv@v@EstRsqBenchpressTolTightMiKfive}{\ensuremath{-}0.042}
\@namedef{nv@v@EstRsqBenchpressTolTightRandomKfive}{0.083}
\@namedef{nv@v@EstRsqBenchpressTolTightTraceKfive}{\ensuremath{-}0.159}
\@namedef{nv@v@EstRsqMergedAlphaPointThreeFaclocKfive}{0.583}
\@namedef{nv@v@EstRsqMergedAlphaPointThreeMiKfive}{0.456}
\@namedef{nv@v@EstRsqMergedAlphaPointThreeRandomKfive}{0.522}
\@namedef{nv@v@EstRsqMergedAlphaPointThreeTraceKfive}{0.572}
\@namedef{nv@v@EstRsqMergedDefaultFaclocKfive}{0.614}
\@namedef{nv@v@EstRsqMergedDefaultMiKfive}{0.465}
\@namedef{nv@v@EstRsqMergedDefaultRandomKfive}{0.563}
\@namedef{nv@v@EstRsqMergedDefaultTraceKfive}{0.593}
\@namedef{nv@v@EstRsqMergedEligOneFaclocKfive}{0.561}
\@namedef{nv@v@EstRsqMergedEligOneMiKfive}{0.465}
\@namedef{nv@v@EstRsqMergedEligOneRandomKfive}{0.511}
\@namedef{nv@v@EstRsqMergedEligOneTraceKfive}{0.538}
\@namedef{nv@v@EstRsqMergedEligTwoFaclocKfive}{0.561}
\@namedef{nv@v@EstRsqMergedEligTwoMiKfive}{0.465}
\@namedef{nv@v@EstRsqMergedEligTwoRandomKfive}{0.511}
\@namedef{nv@v@EstRsqMergedEligTwoTraceKfive}{0.538}
\@namedef{nv@v@EstRsqMergedPairwiseFaclocKfive}{0.619}
\@namedef{nv@v@EstRsqMergedPairwiseMiKfive}{0.473}
\@namedef{nv@v@EstRsqMergedPairwiseRandomKfive}{0.540}
\@namedef{nv@v@EstRsqMergedPairwiseTraceKfive}{0.614}
\@namedef{nv@v@EstRsqMergedPsdMinusSixFaclocKfive}{0.622}
\@namedef{nv@v@EstRsqMergedPsdMinusSixMiKfive}{0.504}
\@namedef{nv@v@EstRsqMergedPsdMinusSixRandomKfive}{0.565}
\@namedef{nv@v@EstRsqMergedPsdMinusSixTraceKfive}{0.620}
\@namedef{nv@v@EstRsqMergedShrinkFourFaclocKfive}{0.585}
\@namedef{nv@v@EstRsqMergedShrinkFourMiKfive}{0.464}
\@namedef{nv@v@EstRsqMergedShrinkFourRandomKfive}{0.526}
\@namedef{nv@v@EstRsqMergedShrinkFourTraceKfive}{0.572}
\@namedef{nv@v@EstRsqMergedTolLooseFaclocKfive}{0.632}
\@namedef{nv@v@EstRsqMergedTolLooseMiKfive}{0.565}
\@namedef{nv@v@EstRsqMergedTolLooseRandomKfive}{0.571}
\@namedef{nv@v@EstRsqMergedTolLooseTraceKfive}{0.648}
\@namedef{nv@v@EstRsqMmluAlphaPointThreeFaclocKfive}{0.882}
\@namedef{nv@v@EstRsqMmluDefaultFaclocKfive}{0.919}
\@namedef{nv@v@FaclocCoverBenchpressKten}{0.813}
\@namedef{nv@v@FaclocCoverMergedKten}{0.824}
\@namedef{nv@v@FaclocCoverMmluKten}{0.969}
\@namedef{nv@v@FaclocCoverMtebKten}{0.938}
\@namedef{nv@v@FigMechMergedNOmitted}{8}
\@namedef{nv@v@ItemBudgetNItemsOlvOneItems}{28{,}659}
\@namedef{nv@v@NBenchProspOlvTwoSubCutJanTwentyfive}{35}
\@namedef{nv@v@NBenchProspOlvTwoSubMathCutJanTwentyfive}{42}
\@namedef{nv@v@NFamBenchpress}{6}
\@namedef{nv@v@NFamEpoch}{11}
\@namedef{nv@v@NFamHelmClassic}{4}
\@namedef{nv@v@NFamHelmLite}{6}
\@namedef{nv@v@NFamHelmMmlu}{6}
\@namedef{nv@v@NFamMerged}{9}
\@namedef{nv@v@NFamMmlu}{8}
\@namedef{nv@v@NFamMteb}{10}
\@namedef{nv@v@NFamMtebTwothousandtwentysix}{15}
\@namedef{nv@v@NFamOlvOneItems}{5}
\@namedef{nv@v@NFamOlvTwoSub}{9}
\@namedef{nv@v@NTestProspEpochByModelCutJanTwentyfive}{158}
\@namedef{nv@v@NTestProspEpochCutJanTwentyfive}{158}
\@namedef{nv@v@NTestProspEpochCutJanTwentysix}{83}
\@namedef{nv@v@NTestProspEpochCutJulTwentyfive}{113}
\@namedef{nv@v@NTestProspEpochCutJulTwentyfour}{194}
\@namedef{nv@v@NTestProspHelm}{61}
\@namedef{nv@v@NTestProspMteb}{57}
\@namedef{nv@v@NTestProspMtebLate}{36}
\@namedef{nv@v@NTestProspOlvTwoSubCutJanTwentyfive}{1{,}888}
\@namedef{nv@v@NTestProspOlvTwoSubCutMarTwentyfive}{334}
\@namedef{nv@v@NTestProspOlvTwoSubCutOctTwentyfour}{3{,}229}
\@namedef{nv@v@NTestProspOlvTwoSubMathCutJanTwentyfive}{1{,}889}
\@namedef{nv@v@NTrainProspEpochByModelCutJanTwentyfive}{119}
\@namedef{nv@v@NTrainProspEpochCutJanTwentyfive}{119}
\@namedef{nv@v@NTrainProspEpochCutJanTwentysix}{194}
\@namedef{nv@v@NTrainProspEpochCutJulTwentyfive}{164}
\@namedef{nv@v@NTrainProspEpochCutJulTwentyfour}{83}
\@namedef{nv@v@NTrainProspHelm}{30}
\@namedef{nv@v@NTrainProspMteb}{263}
\@namedef{nv@v@NTrainProspMtebLate}{263}
\@namedef{nv@v@NTrainProspOlvTwoSubCutJanTwentyfive}{2{,}593}
\@namedef{nv@v@NTrainProspOlvTwoSubCutMarTwentyfive}{4{,}144}
\@namedef{nv@v@NTrainProspOlvTwoSubCutOctTwentyfour}{1{,}252}
\@namedef{nv@v@NTrainProspOlvTwoSubMathCutJanTwentyfive}{2{,}593}
\@namedef{nv@v@NormMergedN}{114}
\@namedef{nv@v@NormMergedNRejectBh}{60}
\@namedef{nv@v@NormMmluN}{57}
\@namedef{nv@v@NormMmluNRejectBh}{57}
\@namedef{nv@v@NormMtebN}{56}
\@namedef{nv@v@NormMtebNComplete}{133}
\@namedef{nv@v@NormMtebNRejectBh}{56}
\@namedef{nv@v@ObjBruteBenchpressFaclocKthreeFRatio}{0.991}
\@namedef{nv@v@ObjBruteBenchpressFaclocKthreeFRatioMin}{0.968}
\@namedef{nv@v@ObjBruteMergedFaclocKthreeFRatio}{0.988}
\@namedef{nv@v@ObjBruteMergedFaclocKthreeFRatioMin}{0.961}
\@namedef{nv@v@ObjBruteMmluFaclocKthreeFRatio}{1.000}
\@namedef{nv@v@ObjBruteMmluFaclocKthreeFRatioMin}{1.000}
\@namedef{nv@v@ObjBruteMtebFaclocKthreeFRatio}{0.990}
\@namedef{nv@v@ObjBruteMtebFaclocKthreeFRatioMin}{0.987}
\@namedef{nv@v@ObjFirstBenchpressMiRestRsq}{1.000}
\@namedef{nv@v@ObjFirstMergedMiRestRsq}{0.950}
\@namedef{nv@v@ObjFirstMmluMiRestRsq}{0.993}
\@namedef{nv@v@ObjFirstMtebMiRestRsq}{0.997}
\@namedef{nv@v@ObjModalFirstMergedMiSingleRsq}{0.170}
\@namedef{nv@v@ObjModalFirstMergedTraceSingleRsq}{0.533}
\@namedef{nv@v@ObjPopRsqBenchpressTraceKfive}{0.756}
\@namedef{nv@v@ObjPopRsqMmluTraceKfive}{0.921}
\@namedef{nv@v@PairDiffBaseMmluTraceVsFaclocKfive}{0.001}
\@namedef{nv@v@PairDiffBaseMtebFaclocVsRandomKfive}{0.023}
\@namedef{nv@v@PairDiffBaseMtebFaclocVsRandomKone}{0.157}
\@namedef{nv@v@PairNBaseBenchpressFaclocVsRandomKone}{41}
\@namedef{nv@v@PairNBaseMmluTraceVsFaclocKfive}{50}
\@namedef{nv@v@PairNMmluMiVsEntropyKone}{50}
\@namedef{nv@v@PairWinsBaseMmluTraceVsFaclocKfive}{50}
\@namedef{nv@v@PairWinsMmluMiVsEntropyKone}{0}
\@namedef{nv@v@RevClipDatasetsBenchpressMiOutside}{190}
\@namedef{nv@v@RevClipDatasetsBenchpressMiTotal}{4{,}327}
\@namedef{nv@v@RevClipDatasetsMtebTraceOutside}{594}
\@namedef{nv@v@RevClipDatasetsMtebTraceTotal}{51{,}552}
\@namedef{nv@v@RevContamConfigNDraws}{20}
\@namedef{nv@v@RevContamDrawsConfigsFracZeropointthreeDeltaZeropointtwoEntropyRankBefore}{57}
\@namedef{nv@v@RevContamDrawsConfigsFracZeropointthreeDeltaZeropointtwoFaclocRankBefore}{3}
\@namedef{nv@v@RevMonoDatasetsMmluDeterministicFiveRTwoMean}{0.906}
\@namedef{nv@v@RevMonoDatasetsMmluNSteps}{750}
\@namedef{nv@v@RevMonoDatasetsMmluRandomGreedyFiveRTwoMean}{0.902}
\@namedef{nv@v@RsqBaseBenchpressEntropyKfive}{\ensuremath{-}0.300}
\@namedef{nv@v@RsqBaseBenchpressEntropyKone}{\ensuremath{-}0.143}
\@namedef{nv@v@RsqBaseBenchpressEntropyKten}{\ensuremath{-}0.065}
\@namedef{nv@v@RsqBaseBenchpressFaclocKfive}{0.053}
\@namedef{nv@v@RsqBaseBenchpressFaclocKone}{\ensuremath{-}0.033}
\@namedef{nv@v@RsqBaseBenchpressFaclocKten}{0.066}
\@namedef{nv@v@RsqBaseBenchpressHubKfive}{0.032}
\@namedef{nv@v@RsqBaseBenchpressHubKone}{\ensuremath{-}0.071}
\@namedef{nv@v@RsqBaseBenchpressHubKten}{0.035}
\@namedef{nv@v@RsqBaseBenchpressMiKfive}{\ensuremath{-}0.059}
\@namedef{nv@v@RsqBaseBenchpressMiKone}{\ensuremath{-}0.021}
\@namedef{nv@v@RsqBaseBenchpressMiKten}{\ensuremath{-}0.088}
\@namedef{nv@v@RsqBaseBenchpressPcaKfive}{0.060}
\@namedef{nv@v@RsqBaseBenchpressPcaKone}{\ensuremath{-}0.136}
\@namedef{nv@v@RsqBaseBenchpressPcaKten}{\ensuremath{-}0.049}
\@namedef{nv@v@RsqBaseBenchpressRandomKfive}{0.120}
\@namedef{nv@v@RsqBaseBenchpressRandomKone}{0.028}
\@namedef{nv@v@RsqBaseBenchpressRandomKten}{0.207}
\@namedef{nv@v@RsqBaseBenchpressTraceKfive}{\ensuremath{-}0.085}
\@namedef{nv@v@RsqBaseBenchpressTraceKone}{\ensuremath{-}0.143}
\@namedef{nv@v@RsqBaseBenchpressTraceKten}{\ensuremath{-}0.009}
\@namedef{nv@v@RsqBaseEpochEntropyKfive}{0.426}
\@namedef{nv@v@RsqBaseEpochFaclocKfive}{0.475}
\@namedef{nv@v@RsqBaseEpochHubKfive}{0.416}
\@namedef{nv@v@RsqBaseEpochMiKfive}{0.183}
\@namedef{nv@v@RsqBaseEpochPcaKfive}{0.303}
\@namedef{nv@v@RsqBaseEpochRandomKfive}{0.306}
\@namedef{nv@v@RsqBaseEpochTraceKfive}{0.458}
\@namedef{nv@v@RsqBaseHelmClassicEntropyKfive}{0.508}
\@namedef{nv@v@RsqBaseHelmClassicFaclocKfive}{0.541}
\@namedef{nv@v@RsqBaseHelmClassicHubKfive}{0.417}
\@namedef{nv@v@RsqBaseHelmClassicMiKfive}{0.450}
\@namedef{nv@v@RsqBaseHelmClassicPcaKfive}{0.339}
\@namedef{nv@v@RsqBaseHelmClassicRandomKfive}{0.418}
\@namedef{nv@v@RsqBaseHelmClassicTraceKfive}{0.352}
\@namedef{nv@v@RsqBaseHelmLiteEntropyKfive}{0.729}
\@namedef{nv@v@RsqBaseHelmLiteFaclocKfive}{0.719}
\@namedef{nv@v@RsqBaseHelmLiteHubKfive}{0.472}
\@namedef{nv@v@RsqBaseHelmLiteMiKfive}{0.720}
\@namedef{nv@v@RsqBaseHelmLitePcaKfive}{0.661}
\@namedef{nv@v@RsqBaseHelmLiteRandomKfive}{0.669}
\@namedef{nv@v@RsqBaseHelmLiteTraceKfive}{0.727}
\@namedef{nv@v@RsqBaseHelmMmluEntropyKfive}{0.761}
\@namedef{nv@v@RsqBaseHelmMmluFaclocKfive}{0.780}
\@namedef{nv@v@RsqBaseHelmMmluHubKfive}{0.702}
\@namedef{nv@v@RsqBaseHelmMmluMiKfive}{0.774}
\@namedef{nv@v@RsqBaseHelmMmluPcaKfive}{0.759}
\@namedef{nv@v@RsqBaseHelmMmluRandomKfive}{0.740}
\@namedef{nv@v@RsqBaseHelmMmluTraceKfive}{0.786}
\@namedef{nv@v@RsqBaseMergedEntropyKfive}{0.503}
\@namedef{nv@v@RsqBaseMergedEntropyKone}{0.490}
\@namedef{nv@v@RsqBaseMergedEntropyKten}{0.549}
\@namedef{nv@v@RsqBaseMergedFaclocKfive}{0.614}
\@namedef{nv@v@RsqBaseMergedFaclocKone}{0.317}
\@namedef{nv@v@RsqBaseMergedFaclocKten}{0.661}
\@namedef{nv@v@RsqBaseMergedFaclocSqKone}{0.490}
\@namedef{nv@v@RsqBaseMergedHubKfive}{0.481}
\@namedef{nv@v@RsqBaseMergedHubKone}{0.320}
\@namedef{nv@v@RsqBaseMergedHubKten}{0.537}
\@namedef{nv@v@RsqBaseMergedMiKfive}{0.465}
\@namedef{nv@v@RsqBaseMergedMiKone}{0.084}
\@namedef{nv@v@RsqBaseMergedMiKten}{0.528}
\@namedef{nv@v@RsqBaseMergedPcaKfive}{0.483}
\@namedef{nv@v@RsqBaseMergedPcaKone}{0.489}
\@namedef{nv@v@RsqBaseMergedPcaKten}{0.539}
\@namedef{nv@v@RsqBaseMergedRandomKfive}{0.563}
\@namedef{nv@v@RsqBaseMergedRandomKone}{0.260}
\@namedef{nv@v@RsqBaseMergedRandomKten}{0.604}
\@namedef{nv@v@RsqBaseMergedTraceKfive}{0.593}
\@namedef{nv@v@RsqBaseMergedTraceKone}{0.490}
\@namedef{nv@v@RsqBaseMergedTraceKten}{0.626}
\@namedef{nv@v@RsqBaseMergedVOneEntropyKfive}{0.514}
\@namedef{nv@v@RsqBaseMergedVOneFaclocKfive}{0.619}
\@namedef{nv@v@RsqBaseMergedVOneHubKfive}{0.466}
\@namedef{nv@v@RsqBaseMergedVOneMiKfive}{0.486}
\@namedef{nv@v@RsqBaseMergedVOnePcaKfive}{0.471}
\@namedef{nv@v@RsqBaseMergedVOneRandomKfive}{0.564}
\@namedef{nv@v@RsqBaseMergedVOneTraceKfive}{0.596}
\@namedef{nv@v@RsqBaseMmluEntropyKfive}{0.913}
\@namedef{nv@v@RsqBaseMmluEntropyKone}{0.860}
\@namedef{nv@v@RsqBaseMmluEntropyKten}{0.936}
\@namedef{nv@v@RsqBaseMmluFaclocKfive}{0.919}
\@namedef{nv@v@RsqBaseMmluFaclocKone}{0.860}
\@namedef{nv@v@RsqBaseMmluFaclocKten}{0.945}
\@namedef{nv@v@RsqBaseMmluHubKfive}{0.875}
\@namedef{nv@v@RsqBaseMmluHubKone}{0.860}
\@namedef{nv@v@RsqBaseMmluHubKten}{0.886}
\@namedef{nv@v@RsqBaseMmluMiKfive}{0.906}
\@namedef{nv@v@RsqBaseMmluMiKone}{0.832}
\@namedef{nv@v@RsqBaseMmluMiKten}{0.911}
\@namedef{nv@v@RsqBaseMmluPcaKfive}{0.907}
\@namedef{nv@v@RsqBaseMmluPcaKone}{0.860}
\@namedef{nv@v@RsqBaseMmluPcaKten}{0.940}
\@namedef{nv@v@RsqBaseMmluRandomKfive}{0.890}
\@namedef{nv@v@RsqBaseMmluRandomKone}{0.751}
\@namedef{nv@v@RsqBaseMmluRandomKten}{0.911}
\@namedef{nv@v@RsqBaseMmluTraceKfive}{0.920}
\@namedef{nv@v@RsqBaseMmluTraceKone}{0.860}
\@namedef{nv@v@RsqBaseMmluTraceKten}{0.946}
\@namedef{nv@v@RsqBaseMtebEntropyKfive}{0.746}
\@namedef{nv@v@RsqBaseMtebEntropyKone}{0.646}
\@namedef{nv@v@RsqBaseMtebEntropyKten}{0.817}
\@namedef{nv@v@RsqBaseMtebFaclocKfive}{0.767}
\@namedef{nv@v@RsqBaseMtebFaclocKone}{0.659}
\@namedef{nv@v@RsqBaseMtebFaclocKten}{0.826}
\@namedef{nv@v@RsqBaseMtebHubKfive}{0.687}
\@namedef{nv@v@RsqBaseMtebHubKone}{0.659}
\@namedef{nv@v@RsqBaseMtebHubKten}{0.718}
\@namedef{nv@v@RsqBaseMtebMiKfive}{0.767}
\@namedef{nv@v@RsqBaseMtebMiKone}{0.650}
\@namedef{nv@v@RsqBaseMtebMiKten}{0.821}
\@namedef{nv@v@RsqBaseMtebPcaKfive}{0.755}
\@namedef{nv@v@RsqBaseMtebPcaKone}{0.648}
\@namedef{nv@v@RsqBaseMtebPcaKten}{0.801}
\@namedef{nv@v@RsqBaseMtebRandomKfive}{0.744}
\@namedef{nv@v@RsqBaseMtebRandomKone}{0.502}
\@namedef{nv@v@RsqBaseMtebRandomKten}{0.784}
\@namedef{nv@v@RsqBaseMtebTraceKfive}{0.790}
\@namedef{nv@v@RsqBaseMtebTraceKone}{0.646}
\@namedef{nv@v@RsqBaseMtebTraceKten}{0.839}
\@namedef{nv@v@RsqBaseMtebTwothousandtwentysixEntropyKfive}{0.720}
\@namedef{nv@v@RsqBaseMtebTwothousandtwentysixFaclocKfive}{0.764}
\@namedef{nv@v@RsqBaseMtebTwothousandtwentysixHubKfive}{0.651}
\@namedef{nv@v@RsqBaseMtebTwothousandtwentysixMiKfive}{0.752}
\@namedef{nv@v@RsqBaseMtebTwothousandtwentysixPcaKfive}{0.716}
\@namedef{nv@v@RsqBaseMtebTwothousandtwentysixRandomKfive}{0.710}
\@namedef{nv@v@RsqBaseMtebTwothousandtwentysixTraceKfive}{0.752}
\@namedef{nv@v@RsqBaseOlvOneItemsEntropyKfive}{0.832}
\@namedef{nv@v@RsqBaseOlvOneItemsFaclocKfive}{0.844}
\@namedef{nv@v@RsqBaseOlvOneItemsHubKfive}{0.795}
\@namedef{nv@v@RsqBaseOlvOneItemsMiKfive}{0.838}
\@namedef{nv@v@RsqBaseOlvOneItemsPcaKfive}{0.801}
\@namedef{nv@v@RsqBaseOlvOneItemsRandomKfive}{0.813}
\@namedef{nv@v@RsqBaseOlvOneItemsTraceKfive}{0.845}
\@namedef{nv@v@RsqBaseOlvTwoSubEntropyKfive}{0.649}
\@namedef{nv@v@RsqBaseOlvTwoSubFaclocKfive}{0.736}
\@namedef{nv@v@RsqBaseOlvTwoSubHubKfive}{0.570}
\@namedef{nv@v@RsqBaseOlvTwoSubMiKfive}{0.680}
\@namedef{nv@v@RsqBaseOlvTwoSubPcaKfive}{0.706}
\@namedef{nv@v@RsqBaseOlvTwoSubRandomKfive}{0.643}
\@namedef{nv@v@RsqBaseOlvTwoSubTraceKfive}{0.738}
\@namedef{nv@v@RsqBenchpressEntropyKfivePninety}{0.105}
\@namedef{nv@v@RsqBenchpressFaclocKfivePninety}{0.095}
\@namedef{nv@v@RsqBenchpressRandomKfivePninety}{0.106}
\@namedef{nv@v@RsqBenchpressTraceKfivePninety}{0.114}
\@namedef{nv@v@RsqCenProspEpochCutJanTwentyfiveFaclocKfive}{\ensuremath{-}0.963}
\@namedef{nv@v@RsqCenProspHelmFaclocKfive}{0.371}
\@namedef{nv@v@RsqCenProspHelmTraceKfive}{0.316}
\@namedef{nv@v@RsqCenProspMtebFaclocKfive}{0.515}
\@namedef{nv@v@RsqCenProspMtebHubKfive}{0.225}
\@namedef{nv@v@RsqCenProspMtebLateFaclocKfive}{0.617}
\@namedef{nv@v@RsqCenProspMtebLatePcaKfive}{0.631}
\@namedef{nv@v@RsqCenProspMtebLateTraceKfive}{0.677}
\@namedef{nv@v@RsqCenProspMtebTraceKfive}{0.466}
\@namedef{nv@v@RsqCtrlEpochByModelCutJanTwentyfiveFaclocKfive}{0.366}
\@namedef{nv@v@RsqCtrlEpochCutJanTwentyfiveFaclocKfive}{0.409}
\@namedef{nv@v@RsqCtrlEpochCutJanTwentysixFaclocKfive}{0.408}
\@namedef{nv@v@RsqCtrlEpochCutJulTwentyfiveFaclocKfive}{0.417}
\@namedef{nv@v@RsqCtrlEpochCutJulTwentyfourFaclocKfive}{0.365}
\@namedef{nv@v@RsqCtrlHelmFaclocKfive}{0.694}
\@namedef{nv@v@RsqCtrlMtebFaclocKfive}{0.784}
\@namedef{nv@v@RsqCtrlMtebLateFaclocKfive}{0.789}
\@namedef{nv@v@RsqCtrlOlvTwoSubCutJanTwentyfiveFaclocKfive}{0.698}
\@namedef{nv@v@RsqCtrlOlvTwoSubCutMarTwentyfiveFaclocKfive}{0.698}
\@namedef{nv@v@RsqCtrlOlvTwoSubCutOctTwentyfourFaclocKfive}{0.700}
\@namedef{nv@v@RsqCtrlOlvTwoSubMathCutJanTwentyfiveFaclocKfive}{0.735}
\@namedef{nv@v@RsqEpochEntropyKfivePninety}{0.166}
\@namedef{nv@v@RsqEpochFaclocKfivePninety}{0.214}
\@namedef{nv@v@RsqEpochRandomKfivePninety}{0.176}
\@namedef{nv@v@RsqEpochTraceKfivePninety}{0.199}
\@namedef{nv@v@RsqFamBenchpressEntropyKfive}{0.052}
\@namedef{nv@v@RsqFamBenchpressFaclocKfive}{0.053}
\@namedef{nv@v@RsqFamBenchpressFaclocKfiveClaude}{\ensuremath{-}0.129}
\@namedef{nv@v@RsqFamBenchpressFaclocKfiveDeepseek}{0.180}
\@namedef{nv@v@RsqFamBenchpressFaclocKfiveGemini}{0.301}
\@namedef{nv@v@RsqFamBenchpressFaclocKfiveGpt}{0.121}
\@namedef{nv@v@RsqFamBenchpressFaclocKfiveLlama}{\ensuremath{-}0.264}
\@namedef{nv@v@RsqFamBenchpressFaclocKfiveQwen}{0.109}
\@namedef{nv@v@RsqFamBenchpressHubKfive}{0.016}
\@namedef{nv@v@RsqFamBenchpressMiKfive}{\ensuremath{-}0.332}
\@namedef{nv@v@RsqFamBenchpressPcaKfive}{\ensuremath{-}0.085}
\@namedef{nv@v@RsqFamBenchpressRandomKfive}{0.170}
\@namedef{nv@v@RsqFamEpochEntropyKfive}{0.342}
\@namedef{nv@v@RsqFamEpochFaclocKfive}{0.369}
\@namedef{nv@v@RsqFamEpochHubKfive}{0.260}
\@namedef{nv@v@RsqFamEpochMiKfive}{\ensuremath{-}0.141}
\@namedef{nv@v@RsqFamEpochPcaKfive}{0.259}
\@namedef{nv@v@RsqFamEpochRandomKfive}{0.196}
\@namedef{nv@v@RsqFamEpochTraceKfive}{0.336}
\@namedef{nv@v@RsqFamHelmClassicEntropyKfive}{0.619}
\@namedef{nv@v@RsqFamHelmClassicFaclocKfive}{0.683}
\@namedef{nv@v@RsqFamHelmClassicHubKfive}{0.436}
\@namedef{nv@v@RsqFamHelmClassicMiKfive}{0.648}
\@namedef{nv@v@RsqFamHelmClassicPcaKfive}{0.644}
\@namedef{nv@v@RsqFamHelmClassicRandomKfive}{0.545}
\@namedef{nv@v@RsqFamHelmClassicTraceKfive}{0.663}
\@namedef{nv@v@RsqFamHelmLiteEntropyKfive}{0.412}
\@namedef{nv@v@RsqFamHelmLiteFaclocKfive}{0.382}
\@namedef{nv@v@RsqFamHelmLiteHubKfive}{0.327}
\@namedef{nv@v@RsqFamHelmLiteMiKfive}{0.487}
\@namedef{nv@v@RsqFamHelmLitePcaKfive}{0.355}
\@namedef{nv@v@RsqFamHelmLiteRandomKfive}{0.471}
\@namedef{nv@v@RsqFamHelmLiteTraceKfive}{0.412}
\@namedef{nv@v@RsqFamHelmMmluEntropyKfive}{0.720}
\@namedef{nv@v@RsqFamHelmMmluFaclocKfive}{0.748}
\@namedef{nv@v@RsqFamHelmMmluHubKfive}{0.680}
\@namedef{nv@v@RsqFamHelmMmluMiKfive}{0.750}
\@namedef{nv@v@RsqFamHelmMmluPcaKfive}{0.725}
\@namedef{nv@v@RsqFamHelmMmluRandomKfive}{0.716}
\@namedef{nv@v@RsqFamHelmMmluTraceKfive}{0.753}
\@namedef{nv@v@RsqFamMergedEntropyKfive}{0.492}
\@namedef{nv@v@RsqFamMergedFaclocKfive}{0.663}
\@namedef{nv@v@RsqFamMergedFaclocKfiveClaude}{0.561}
\@namedef{nv@v@RsqFamMergedFaclocKfiveGemini}{0.572}
\@namedef{nv@v@RsqFamMergedFaclocKfiveGemma}{0.853}
\@namedef{nv@v@RsqFamMergedFaclocKfiveGpt}{0.802}
\@namedef{nv@v@RsqFamMergedFaclocKfiveLlama}{0.673}
\@namedef{nv@v@RsqFamMergedFaclocKfiveMistral}{0.675}
\@namedef{nv@v@RsqFamMergedFaclocKfivePhi}{0.570}
\@namedef{nv@v@RsqFamMergedFaclocKfiveQwen}{0.671}
\@namedef{nv@v@RsqFamMergedFaclocKfiveYi}{0.587}
\@namedef{nv@v@RsqFamMergedHubKfive}{0.596}
\@namedef{nv@v@RsqFamMergedMiKfive}{0.464}
\@namedef{nv@v@RsqFamMergedPcaKfive}{0.504}
\@namedef{nv@v@RsqFamMergedRandomKfive}{0.562}
\@namedef{nv@v@RsqFamMergedTraceKfive}{0.619}
\@namedef{nv@v@RsqFamMmluEntropyKfive}{0.897}
\@namedef{nv@v@RsqFamMmluFaclocKfive}{0.899}
\@namedef{nv@v@RsqFamMmluFaclocKfiveGemma}{0.896}
\@namedef{nv@v@RsqFamMmluFaclocKfiveGpt}{0.957}
\@namedef{nv@v@RsqFamMmluFaclocKfiveLlama}{0.922}
\@namedef{nv@v@RsqFamMmluFaclocKfiveMistral}{0.898}
\@namedef{nv@v@RsqFamMmluFaclocKfivePhi}{0.855}
\@namedef{nv@v@RsqFamMmluFaclocKfiveQwen}{0.917}
\@namedef{nv@v@RsqFamMmluFaclocKfiveSolar}{0.808}
\@namedef{nv@v@RsqFamMmluFaclocKfiveYi}{0.935}
\@namedef{nv@v@RsqFamMmluHubKfive}{0.852}
\@namedef{nv@v@RsqFamMmluMiKfive}{0.890}
\@namedef{nv@v@RsqFamMmluPcaKfive}{0.881}
\@namedef{nv@v@RsqFamMmluRandomKfive}{0.866}
\@namedef{nv@v@RsqFamMmluTraceKfive}{0.903}
\@namedef{nv@v@RsqFamMtebEntropyKfive}{0.560}
\@namedef{nv@v@RsqFamMtebFaclocKfive}{0.621}
\@namedef{nv@v@RsqFamMtebFaclocKfiveAlibabaNlp}{0.801}
\@namedef{nv@v@RsqFamMtebFaclocKfiveBaai}{0.848}
\@namedef{nv@v@RsqFamMtebFaclocKfiveIntfloat}{0.493}
\@namedef{nv@v@RsqFamMtebFaclocKfiveJinaai}{0.318}
\@namedef{nv@v@RsqFamMtebFaclocKfiveMcgillNlp}{0.597}
\@namedef{nv@v@RsqFamMtebFaclocKfiveMihaiii}{0.641}
\@namedef{nv@v@RsqFamMtebFaclocKfiveMinishlab}{0.868}
\@namedef{nv@v@RsqFamMtebFaclocKfiveSentenceTransformers}{0.617}
\@namedef{nv@v@RsqFamMtebFaclocKfiveSnowflake}{0.411}
\@namedef{nv@v@RsqFamMtebFaclocKfiveVoyageai}{0.610}
\@namedef{nv@v@RsqFamMtebHubKfive}{0.500}
\@namedef{nv@v@RsqFamMtebMiKfive}{0.572}
\@namedef{nv@v@RsqFamMtebPcaKfive}{0.542}
\@namedef{nv@v@RsqFamMtebRandomKfive}{0.550}
\@namedef{nv@v@RsqFamMtebTraceKfive}{0.620}
\@namedef{nv@v@RsqFamMtebTwothousandtwentysixEntropyKfive}{0.520}
\@namedef{nv@v@RsqFamMtebTwothousandtwentysixFaclocKfive}{0.602}
\@namedef{nv@v@RsqFamMtebTwothousandtwentysixHubKfive}{0.424}
\@namedef{nv@v@RsqFamMtebTwothousandtwentysixMiKfive}{0.542}
\@namedef{nv@v@RsqFamMtebTwothousandtwentysixPcaKfive}{0.489}
\@namedef{nv@v@RsqFamMtebTwothousandtwentysixRandomKfive}{0.541}
\@namedef{nv@v@RsqFamMtebTwothousandtwentysixTraceKfive}{0.606}
\@namedef{nv@v@RsqFamOlvOneItemsEntropyKfive}{0.837}
\@namedef{nv@v@RsqFamOlvOneItemsFaclocKfive}{0.822}
\@namedef{nv@v@RsqFamOlvOneItemsHubKfive}{0.788}
\@namedef{nv@v@RsqFamOlvOneItemsMiKfive}{0.819}
\@namedef{nv@v@RsqFamOlvOneItemsPcaKfive}{0.778}
\@namedef{nv@v@RsqFamOlvOneItemsRandomKfive}{0.786}
\@namedef{nv@v@RsqFamOlvOneItemsTraceKfive}{0.829}
\@namedef{nv@v@RsqFamOlvTwoSubEntropyKfive}{0.592}
\@namedef{nv@v@RsqFamOlvTwoSubFaclocKfive}{0.726}
\@namedef{nv@v@RsqFamOlvTwoSubHubKfive}{0.515}
\@namedef{nv@v@RsqFamOlvTwoSubMiKfive}{0.637}
\@namedef{nv@v@RsqFamOlvTwoSubPcaKfive}{0.644}
\@namedef{nv@v@RsqFamOlvTwoSubRandomKfive}{0.607}
\@namedef{nv@v@RsqFamOlvTwoSubTraceKfive}{0.717}
\@namedef{nv@v@RsqImpGaussBenchpressFaclocKfive}{0.053}
\@namedef{nv@v@RsqImpGaussBenchpressHubKfive}{0.032}
\@namedef{nv@v@RsqImpGaussBenchpressMiKfive}{\ensuremath{-}0.059}
\@namedef{nv@v@RsqImpGaussBenchpressRandomKfive}{0.120}
\@namedef{nv@v@RsqImpGaussBenchpressTraceKfive}{\ensuremath{-}0.085}
\@namedef{nv@v@RsqImpGaussMergedFaclocKfive}{0.614}
\@namedef{nv@v@RsqImpGaussMergedHubKfive}{0.481}
\@namedef{nv@v@RsqImpGaussMergedMiKfive}{0.465}
\@namedef{nv@v@RsqImpGaussMergedRandomKfive}{0.563}
\@namedef{nv@v@RsqImpGaussMergedTraceKfive}{0.593}
\@namedef{nv@v@RsqImpGaussMmluFaclocKfive}{0.919}
\@namedef{nv@v@RsqImpGaussMmluHubKfive}{0.875}
\@namedef{nv@v@RsqImpGaussMmluMiKfive}{0.906}
\@namedef{nv@v@RsqImpGaussMmluRandomKfive}{0.890}
\@namedef{nv@v@RsqImpGaussMmluTraceKfive}{0.920}
\@namedef{nv@v@RsqImpGaussMtebFaclocKfive}{0.767}
\@namedef{nv@v@RsqImpGaussMtebHubKfive}{0.687}
\@namedef{nv@v@RsqImpGaussMtebMiKfive}{0.767}
\@namedef{nv@v@RsqImpGaussMtebRandomKfive}{0.744}
\@namedef{nv@v@RsqImpGaussMtebTraceKfive}{0.790}
\@namedef{nv@v@RsqImpHardBenchpressFaclocKfive}{0.022}
\@namedef{nv@v@RsqImpHardBenchpressHubKfive}{0.170}
\@namedef{nv@v@RsqImpHardBenchpressMiKfive}{\ensuremath{-}0.148}
\@namedef{nv@v@RsqImpHardBenchpressRandomKfive}{0.049}
\@namedef{nv@v@RsqImpHardBenchpressTraceKfive}{\ensuremath{-}0.144}
\@namedef{nv@v@RsqImpHardMergedFaclocKfive}{0.564}
\@namedef{nv@v@RsqImpHardMergedHubKfive}{0.301}
\@namedef{nv@v@RsqImpHardMergedMiKfive}{0.271}
\@namedef{nv@v@RsqImpHardMergedRandomKfive}{0.398}
\@namedef{nv@v@RsqImpHardMergedTraceKfive}{0.514}
\@namedef{nv@v@RsqImpHardMmluFaclocKfive}{0.900}
\@namedef{nv@v@RsqImpHardMmluHubKfive}{0.859}
\@namedef{nv@v@RsqImpHardMmluMiKfive}{0.892}
\@namedef{nv@v@RsqImpHardMmluRandomKfive}{0.866}
\@namedef{nv@v@RsqImpHardMmluTraceKfive}{0.900}
\@namedef{nv@v@RsqImpHardMtebFaclocKfive}{0.716}
\@namedef{nv@v@RsqImpHardMtebHubKfive}{0.666}
\@namedef{nv@v@RsqImpHardMtebMiKfive}{0.684}
\@namedef{nv@v@RsqImpHardMtebRandomKfive}{0.670}
\@namedef{nv@v@RsqImpHardMtebTraceKfive}{0.735}
\@namedef{nv@v@RsqImpSoftBenchpressFaclocKfive}{0.179}
\@namedef{nv@v@RsqImpSoftBenchpressHubKfive}{0.243}
\@namedef{nv@v@RsqImpSoftBenchpressMiKfive}{0.135}
\@namedef{nv@v@RsqImpSoftBenchpressRandomKfive}{0.193}
\@namedef{nv@v@RsqImpSoftBenchpressTraceKfive}{0.132}
\@namedef{nv@v@RsqImpSoftMergedFaclocKfive}{0.448}
\@namedef{nv@v@RsqImpSoftMergedHubKfive}{0.384}
\@namedef{nv@v@RsqImpSoftMergedMiKfive}{0.302}
\@namedef{nv@v@RsqImpSoftMergedRandomKfive}{0.389}
\@namedef{nv@v@RsqImpSoftMergedTraceKfive}{0.428}
\@namedef{nv@v@RsqImpSoftMmluFaclocKfive}{0.792}
\@namedef{nv@v@RsqImpSoftMmluHubKfive}{0.809}
\@namedef{nv@v@RsqImpSoftMmluMiKfive}{0.836}
\@namedef{nv@v@RsqImpSoftMmluRandomKfive}{0.786}
\@namedef{nv@v@RsqImpSoftMmluTraceKfive}{0.788}
\@namedef{nv@v@RsqImpSoftMtebFaclocKfive}{0.691}
\@namedef{nv@v@RsqImpSoftMtebHubKfive}{0.631}
\@namedef{nv@v@RsqImpSoftMtebMiKfive}{0.657}
\@namedef{nv@v@RsqImpSoftMtebRandomKfive}{0.614}
\@namedef{nv@v@RsqImpSoftMtebTraceKfive}{0.671}
\@namedef{nv@v@RsqLogitBenchpressEntropyKfive}{\ensuremath{-}0.032}
\@namedef{nv@v@RsqLogitMergedFaclocKfive}{0.486}
\@namedef{nv@v@RsqMergedEntropyKfivePninety}{0.114}
\@namedef{nv@v@RsqMergedFaclocKfivePninety}{0.137}
\@namedef{nv@v@RsqMergedRandomKfivePninety}{0.142}
\@namedef{nv@v@RsqMergedTraceKfivePninety}{0.146}
\@namedef{nv@v@RsqMmluEntropyKfivePninety}{0.912}
\@namedef{nv@v@RsqMmluFaclocKfivePninety}{0.918}
\@namedef{nv@v@RsqMmluRandomKfivePninety}{0.891}
\@namedef{nv@v@RsqMmluTraceKfivePninety}{0.919}
\@namedef{nv@v@RsqMtebEntropyKfivePninety}{0.618}
\@namedef{nv@v@RsqMtebFaclocKfivePninety}{0.642}
\@namedef{nv@v@RsqMtebRandomKfivePninety}{0.625}
\@namedef{nv@v@RsqMtebTraceKfivePninety}{0.653}
\@namedef{nv@v@RsqMtebTwothousandtwentysixEntropyKfivePninety}{0.639}
\@namedef{nv@v@RsqMtebTwothousandtwentysixFaclocKfivePninety}{0.645}
\@namedef{nv@v@RsqMtebTwothousandtwentysixRandomKfivePninety}{0.623}
\@namedef{nv@v@RsqMtebTwothousandtwentysixTraceKfivePninety}{0.656}
\@namedef{nv@v@RsqOlvTwoSubEntropyKfivePninety}{0.644}
\@namedef{nv@v@RsqOlvTwoSubFaclocKfivePninety}{0.735}
\@namedef{nv@v@RsqOlvTwoSubRandomKfivePninety}{0.636}
\@namedef{nv@v@RsqOlvTwoSubTraceKfivePninety}{0.735}
\@namedef{nv@v@RsqProspEpochByModelCutJanTwentyfiveEntropyKfive}{0.642}
\@namedef{nv@v@RsqProspEpochByModelCutJanTwentyfiveFaclocKfive}{0.633}
\@namedef{nv@v@RsqProspEpochByModelCutJanTwentyfiveHubKfive}{0.673}
\@namedef{nv@v@RsqProspEpochByModelCutJanTwentyfiveMiKfive}{0.518}
\@namedef{nv@v@RsqProspEpochByModelCutJanTwentyfivePcaKfive}{0.366}
\@namedef{nv@v@RsqProspEpochByModelCutJanTwentyfiveRandomKfive}{0.512}
\@namedef{nv@v@RsqProspEpochByModelCutJanTwentyfiveTraceKfive}{0.658}
\@namedef{nv@v@RsqProspEpochCutJanTwentyfiveEntropyKfive}{0.745}
\@namedef{nv@v@RsqProspEpochCutJanTwentyfiveFaclocKfive}{0.635}
\@namedef{nv@v@RsqProspEpochCutJanTwentyfiveHubKfive}{0.635}
\@namedef{nv@v@RsqProspEpochCutJanTwentyfiveMiKfive}{0.627}
\@namedef{nv@v@RsqProspEpochCutJanTwentyfivePcaKfive}{0.661}
\@namedef{nv@v@RsqProspEpochCutJanTwentyfiveRandomKfive}{0.511}
\@namedef{nv@v@RsqProspEpochCutJanTwentyfiveTraceKfive}{0.682}
\@namedef{nv@v@RsqProspEpochCutJanTwentysixEntropyKfive}{0.356}
\@namedef{nv@v@RsqProspEpochCutJanTwentysixFaclocKfive}{0.441}
\@namedef{nv@v@RsqProspEpochCutJanTwentysixHubKfive}{0.290}
\@namedef{nv@v@RsqProspEpochCutJanTwentysixMiKfive}{0.359}
\@namedef{nv@v@RsqProspEpochCutJanTwentysixRandomKfive}{0.410}
\@namedef{nv@v@RsqProspEpochCutJanTwentysixTraceKfive}{0.719}
\@namedef{nv@v@RsqProspEpochCutJulTwentyfiveEntropyKfive}{0.374}
\@namedef{nv@v@RsqProspEpochCutJulTwentyfiveFaclocKfive}{0.462}
\@namedef{nv@v@RsqProspEpochCutJulTwentyfiveHubKfive}{0.243}
\@namedef{nv@v@RsqProspEpochCutJulTwentyfiveMiKfive}{0.278}
\@namedef{nv@v@RsqProspEpochCutJulTwentyfivePcaKfive}{0.202}
\@namedef{nv@v@RsqProspEpochCutJulTwentyfiveRandomKfive}{0.341}
\@namedef{nv@v@RsqProspEpochCutJulTwentyfiveTraceKfive}{0.481}
\@namedef{nv@v@RsqProspEpochCutJulTwentyfourEntropyKfive}{0.891}
\@namedef{nv@v@RsqProspEpochCutJulTwentyfourFaclocKfive}{0.882}
\@namedef{nv@v@RsqProspEpochCutJulTwentyfourHubKfive}{0.148}
\@namedef{nv@v@RsqProspEpochCutJulTwentyfourMiKfive}{0.329}
\@namedef{nv@v@RsqProspEpochCutJulTwentyfourPcaKfive}{0.375}
\@namedef{nv@v@RsqProspEpochCutJulTwentyfourRandomKfive}{0.588}
\@namedef{nv@v@RsqProspEpochCutJulTwentyfourTraceKfive}{0.286}
\@namedef{nv@v@RsqProspHelmEntropyKfive}{0.581}
\@namedef{nv@v@RsqProspHelmFaclocKfive}{0.718}
\@namedef{nv@v@RsqProspHelmHubKfive}{0.145}
\@namedef{nv@v@RsqProspHelmMiKfive}{0.509}
\@namedef{nv@v@RsqProspHelmPcaKfive}{0.586}
\@namedef{nv@v@RsqProspHelmRandomKfive}{0.382}
\@namedef{nv@v@RsqProspHelmTraceKfive}{0.581}
\@namedef{nv@v@RsqProspMtebEntropyKfive}{0.674}
\@namedef{nv@v@RsqProspMtebFaclocKfive}{0.734}
\@namedef{nv@v@RsqProspMtebHubKfive}{0.751}
\@namedef{nv@v@RsqProspMtebLateEntropyKfive}{0.660}
\@namedef{nv@v@RsqProspMtebLateFaclocKfive}{0.731}
\@namedef{nv@v@RsqProspMtebLateHubKfive}{0.595}
\@namedef{nv@v@RsqProspMtebLateMiKfive}{0.676}
\@namedef{nv@v@RsqProspMtebLatePcaKfive}{0.728}
\@namedef{nv@v@RsqProspMtebLateRandomKfive}{0.661}
\@namedef{nv@v@RsqProspMtebLateTraceKfive}{0.764}
\@namedef{nv@v@RsqProspMtebMiKfive}{0.457}
\@namedef{nv@v@RsqProspMtebPcaKfive}{0.681}
\@namedef{nv@v@RsqProspMtebRandomKfive}{0.647}
\@namedef{nv@v@RsqProspMtebTraceKfive}{0.727}
\@namedef{nv@v@RsqProspOlvTwoSubCutJanTwentyfiveEntropyKfive}{0.690}
\@namedef{nv@v@RsqProspOlvTwoSubCutJanTwentyfiveFaclocKfive}{0.736}
\@namedef{nv@v@RsqProspOlvTwoSubCutJanTwentyfiveHubKfive}{0.597}
\@namedef{nv@v@RsqProspOlvTwoSubCutJanTwentyfiveMiKfive}{0.706}
\@namedef{nv@v@RsqProspOlvTwoSubCutJanTwentyfivePcaKfive}{0.681}
\@namedef{nv@v@RsqProspOlvTwoSubCutJanTwentyfiveRandomKfive}{0.655}
\@namedef{nv@v@RsqProspOlvTwoSubCutJanTwentyfiveTraceKfive}{0.723}
\@namedef{nv@v@RsqProspOlvTwoSubCutMarTwentyfiveEntropyKfive}{0.745}
\@namedef{nv@v@RsqProspOlvTwoSubCutMarTwentyfiveFaclocKfive}{0.765}
\@namedef{nv@v@RsqProspOlvTwoSubCutMarTwentyfiveHubKfive}{0.628}
\@namedef{nv@v@RsqProspOlvTwoSubCutMarTwentyfiveMiKfive}{0.740}
\@namedef{nv@v@RsqProspOlvTwoSubCutMarTwentyfivePcaKfive}{0.738}
\@namedef{nv@v@RsqProspOlvTwoSubCutMarTwentyfiveRandomKfive}{0.695}
\@namedef{nv@v@RsqProspOlvTwoSubCutMarTwentyfiveTraceKfive}{0.763}
\@namedef{nv@v@RsqProspOlvTwoSubCutOctTwentyfourEntropyKfive}{0.673}
\@namedef{nv@v@RsqProspOlvTwoSubCutOctTwentyfourFaclocKfive}{0.717}
\@namedef{nv@v@RsqProspOlvTwoSubCutOctTwentyfourHubKfive}{0.585}
\@namedef{nv@v@RsqProspOlvTwoSubCutOctTwentyfourMiKfive}{0.692}
\@namedef{nv@v@RsqProspOlvTwoSubCutOctTwentyfourPcaKfive}{0.664}
\@namedef{nv@v@RsqProspOlvTwoSubCutOctTwentyfourRandomKfive}{0.642}
\@namedef{nv@v@RsqProspOlvTwoSubCutOctTwentyfourTraceKfive}{0.716}
\@namedef{nv@v@RsqProspOlvTwoSubMathCutJanTwentyfiveEntropyKfive}{0.656}
\@namedef{nv@v@RsqProspOlvTwoSubMathCutJanTwentyfiveFaclocKfive}{0.779}
\@namedef{nv@v@RsqProspOlvTwoSubMathCutJanTwentyfiveHubKfive}{0.577}
\@namedef{nv@v@RsqProspOlvTwoSubMathCutJanTwentyfiveMiKfive}{0.723}
\@namedef{nv@v@RsqProspOlvTwoSubMathCutJanTwentyfivePcaKfive}{0.747}
\@namedef{nv@v@RsqProspOlvTwoSubMathCutJanTwentyfiveRandomKfive}{0.672}
\@namedef{nv@v@RsqProspOlvTwoSubMathCutJanTwentyfiveTraceKfive}{0.774}
\@namedef{nv@v@RsqTabMergedFaclocKfive}{0.060}
\@namedef{nv@v@RsqTabMmluFaclocKfive}{0.539}
\@namedef{nv@v@RsqTabMtebFaclocKfive}{0.337}
\@namedef{nv@v@ScoreAllKFaclocVsTraceMaxDeficit}{0.006}
\@namedef{nv@v@ScoreAllKFaclocVsTraceSigWorse}{22}
\@namedef{nv@v@ScoreAllKNCells}{144}
\@namedef{nv@v@ScoreFaclocVsEntropyNotSig}{17}
\@namedef{nv@v@ScoreFaclocVsEntropySigBetter}{15}
\@namedef{nv@v@ScoreFaclocVsEntropySigWorse}{0}
\@namedef{nv@v@ScoreFaclocVsHubNotSig}{10}
\@namedef{nv@v@ScoreFaclocVsHubSigBetter}{22}
\@namedef{nv@v@ScoreFaclocVsHubSigWorse}{0}
\@namedef{nv@v@ScoreFaclocVsMiNotSig}{17}
\@namedef{nv@v@ScoreFaclocVsMiSigBetter}{15}
\@namedef{nv@v@ScoreFaclocVsMiSigWorse}{0}
\@namedef{nv@v@ScoreFaclocVsPcaNotSig}{15}
\@namedef{nv@v@ScoreFaclocVsPcaSigBetter}{17}
\@namedef{nv@v@ScoreFaclocVsPcaSigWorse}{0}
\@namedef{nv@v@ScoreFaclocVsRandomNotSig}{16}
\@namedef{nv@v@ScoreFaclocVsRandomSigBetter}{16}
\@namedef{nv@v@ScoreFaclocVsRandomSigWorse}{0}
\@namedef{nv@v@ScoreFaclocVsTraceMaxDeficit}{0.005}
\@namedef{nv@v@ScoreFaclocVsTraceNotSig}{26}
\@namedef{nv@v@ScoreFaclocVsTraceSigBetter}{0}
\@namedef{nv@v@ScoreFaclocVsTraceSigWorse}{6}
\@namedef{nv@v@ScoreMiVsEntropySigBetter}{3}
\@namedef{nv@v@ScoreMiVsEntropySigWorse}{7}
\@namedef{nv@v@ScoreNCells}{32}
\@namedef{nv@v@ScoreNMatrices}{11}
\@namedef{nv@v@SelMergedMiPtenFirstFolds}{48}
\@namedef{nv@v@SelMmluFaclocKfiveSameSplits}{50}
\@namedef{nv@v@SelMmluTraceKfiveSharedWithFacloc}{4}
\@namedef{nv@v@StabNSubMerged}{10}
\@namedef{nv@v@TieFaclocSplitsBenchpressKten}{25}
\@namedef{nv@v@TieFaclocSplitsMergedKten}{24}
\@namedef{nv@v@TieFaclocSplitsMmluKten}{0}
\@namedef{nv@v@TieFaclocSplitsMtebKten}{46}
\makeatother


==> cr/tables/tab_main_body.tex <==
%
%
%
%
%
\MMLU & 1 & \textbf{\nv{RsqBaseMmluFaclocKone}} & \textbf{\nv{RsqBaseMmluTraceKone}} & \nv{RsqBaseMmluMiKone}$^{\triangledown}$ & \textbf{\nv{RsqBaseMmluEntropyKone}} & \textbf{\nv{RsqBaseMmluHubKone}} & \textbf{\nv{RsqBaseMmluPcaKone}} & \nv{RsqBaseMmluRandomKone}$^{\triangledown}$ \\
 & 5 & \nv{RsqBaseMmluFaclocKfive} & \textbf{\nv{RsqBaseMmluTraceKfive}}$^{\blacktriangle}$ & \nv{RsqBaseMmluMiKfive}$^{\triangledown}$ & \nv{RsqBaseMmluEntropyKfive}$^{\triangledown}$ & \nv{RsqBaseMmluHubKfive}$^{\triangledown}$ & \nv{RsqBaseMmluPcaKfive}$^{\triangledown}$ & \nv{RsqBaseMmluRandomKfive}$^{\triangledown}$ \\
 & 10 & \nv{RsqBaseMmluFaclocKten} & \textbf{\nv{RsqBaseMmluTraceKten}}$^{\blacktriangle}$ & \nv{RsqBaseMmluMiKten}$^{\triangledown}$ & \nv{RsqBaseMmluEntropyKten}$^{\triangledown}$ & \nv{RsqBaseMmluHubKten}$^{\triangledown}$ & \nv{RsqBaseMmluPcaKten}$^{\triangledown}$ & \nv{RsqBaseMmluRandomKten}$^{\triangledown}$ \\
\addlinespace
\MTEB & 1 & \textbf{\nv{RsqBaseMtebFaclocKone}} & \nv{RsqBaseMtebTraceKone} & \nv{RsqBaseMtebMiKone} & \nv{RsqBaseMtebEntropyKone} & \textbf{\nv{RsqBaseMtebHubKone}} & \nv{RsqBaseMtebPcaKone} & \nv{RsqBaseMtebRandomKone}$^{\triangledown}$ \\
 & 5 & \nv{RsqBaseMtebFaclocKfive} & \textbf{\nv{RsqBaseMtebTraceKfive}} & \nv{RsqBaseMtebMiKfive} & \nv{RsqBaseMtebEntropyKfive} & \nv{RsqBaseMtebHubKfive}$^{\triangledown}$ & \nv{RsqBaseMtebPcaKfive} & \nv{RsqBaseMtebRandomKfive} \\
 & 10 & \nv{RsqBaseMtebFaclocKten} & \textbf{\nv{RsqBaseMtebTraceKten}} & \nv{RsqBaseMtebMiKten} & \nv{RsqBaseMtebEntropyKten} & \nv{RsqBaseMtebHubKten}$^{\triangledown}$ & \nv{RsqBaseMtebPcaKten} & \nv{RsqBaseMtebRandomKten} \\
\addlinespace
\Merged & 1 & \nv{RsqBaseMergedFaclocKone} & \textbf{\nv{RsqBaseMergedTraceKone}} & \nv{RsqBaseMergedMiKone}$^{\dagger}$ & \textbf{\nv{RsqBaseMergedEntropyKone}} & \nv{RsqBaseMergedHubKone} & \nv{RsqBaseMergedPcaKone} & \nv{RsqBaseMergedRandomKone}$^{\dagger}$ \\
 & 5 & \textbf{\nv{RsqBaseMergedFaclocKfive}} & \nv{RsqBaseMergedTraceKfive} & \nv{RsqBaseMergedMiKfive}$^{\triangledown}$ & \nv{RsqBaseMergedEntropyKfive}$^{\triangledown}$ & \nv{RsqBaseMergedHubKfive} & \nv{RsqBaseMergedPcaKfive}$^{\triangledown}$ & \nv{RsqBaseMergedRandomKfive} \\
 & 10 & \textbf{\nv{RsqBaseMergedFaclocKten}} & \nv{RsqBaseMergedTraceKten} & \nv{RsqBaseMergedMiKten}$^{\triangledown}$ & \nv{RsqBaseMergedEntropyKten}$^{\triangledown}$ & \nv{RsqBaseMergedHubKten} & \nv{RsqBaseMergedPcaKten}$^{\triangledown}$ & \nv{RsqBaseMergedRandomKten} \\
\addlinespace
\BenchPress & 1 & \nv{RsqBaseBenchpressFaclocKone} & \nv{RsqBaseBenchpressTraceKone} & \nv{RsqBaseBenchpressMiKone}$^{\dagger}$ & \nv{RsqBaseBenchpressEntropyKone} & \nv{RsqBaseBenchpressHubKone} & \nv{RsqBaseBenchpressPcaKone} & \textbf{\nv{RsqBaseBenchpressRandomKone}}$^{\dagger}$ \\
 & 5 & \nv{RsqBaseBenchpressFaclocKfive} & \nv{RsqBaseBenchpressTraceKfive} & \nv{RsqBaseBenchpressMiKfive}$^{\dagger}$ & \nv{RsqBaseBenchpressEntropyKfive} & \nv{RsqBaseBenchpressHubKfive} & \nv{RsqBaseBenchpressPcaKfive}$^{\dagger}$ & \textbf{\nv{RsqBaseBenchpressRandomKfive}} \\
 & 10 & \nv{RsqBaseBenchpressFaclocKten} & \nv{RsqBaseBenchpressTraceKten} & \nv{RsqBaseBenchpressMiKten} & \nv{RsqBaseBenchpressEntropyKten} & \nv{RsqBaseBenchpressHubKten} & \nv{RsqBaseBenchpressPcaKten} & \textbf{\nv{RsqBaseBenchpressRandomKten}} \\
\midrule
\multicolumn{9}{@{}l}{\emph{Facility location against each column on \nv{ScoreNMatrices} matrices, $k \in \{3, 5, 10\}$ (\nv{ScoreNCells} settings):}} \\
\multicolumn{2}{@{}l}{FL significantly better} & --- & \nv{ScoreFaclocVsTraceSigBetter} & \nv{ScoreFaclocVsMiSigBetter} & \nv{ScoreFaclocVsEntropySigBetter} & \nv{ScoreFaclocVsHubSigBetter} & \nv{ScoreFaclocVsPcaSigBetter} & \nv{ScoreFaclocVsRandomSigBetter} \\
\multicolumn{2}{@{}l}{no significant difference} & --- & \nv{ScoreFaclocVsTraceNotSig} & \nv{ScoreFaclocVsMiNotSig} & \nv{ScoreFaclocVsEntropyNotSig} & \nv{ScoreFaclocVsHubNotSig} & \nv{ScoreFaclocVsPcaNotSig} & \nv{ScoreFaclocVsRandomNotSig} \\
\multicolumn{2}{@{}l}{FL significantly worse} & --- & \nv{ScoreFaclocVsTraceSigWorse} & \nv{ScoreFaclocVsMiSigWorse} & \nv{ScoreFaclocVsEntropySigWorse} & \nv{ScoreFaclocVsHubSigWorse} & \nv{ScoreFaclocVsPcaSigWorse} & \nv{ScoreFaclocVsRandomSigWorse} \\

